Multi-task Representation Learning for Pure Exploration in Bilinear Bandits

We study multi-task representation learning for the problem of pure exploration in bilinear bandits. In bilinear bandits, an action takes the form of a pair of arms from two different entity types and the reward is a bilinear function of the known feature vectors of the arms. In the \textit{multi-task bilinear bandit problem}, we aim to find optimal actions for multiple tasks that share a common low-dimensional linear representation. The objective is to leverage this characteristic to expedite the process of identifying the best pair of arms for all tasks. We propose the algorithm GOBLIN that uses an experimental design approach to optimize sample allocations for learning the global representation as well as minimize the number of samples needed to identify the optimal pair of arms in individual tasks. To the best of our knowledge, this is the first study to give sample complexity analysis for pure exploration in bilinear bandits with shared representation. Our results demonstrate that by learning the shared representation across tasks, we achieve significantly improved sample complexity compared to the traditional approach of solving tasks independently.

==> algo.tex <==




% Algorithm 3 Low Rank Explore Subspace Then Refine (LowESTR)
% 1: Input: arm set $\mathcal{X}$, time horizon $T$, exploration length $T_1$, rank $r$ of $\Theta^*$, spectral bound $\omega_r$ of $\Theta^*$, sampling distribution for stage 1: $D$; parameters for LowOFUL in stage $2: B, B_{\perp}, \lambda, \lambda_{\perp}$.
% 2: Stage 1: Explore the Low Rank Subspace
% 3: Pull $X_t \in \mathcal{X}$ according to distribution $D$ and observe reward $Y_t$, for $t=1, \ldots, T_1$.
% 4: Solve $\hat{\Theta}$ using the problem below:
% \begin{align*}
% \widehat{\Theta}=\operatorname{argmin}_{\Theta \in \mathbb{R}^{d_1 \times d_2}} \frac{1}{2 T_1} \sum_{t=1}^{T_1}\left(Y_t-\left\langle X_t, \Theta\right\rangle\right)^2+\lambda_{T_1}\|\Theta\|_{\mathrm{nuc}} .
% \end{align*}
% 5: Let $\widehat{\Theta}=U \widehat{S} V^T$ be the SVD of $\widehat{\Theta}$. Take the first $r$ columns of $U$ as $\widehat{U}$, the first $r$ rows of $V$ as $\widehat{V}$. Let $\widehat{U}_{\perp}$ and $\widehat{V}_{\perp}$ be orthonormal bases of the complementary subspaces of $\hat{U}$ and $\widehat{V}$.




\begin{algorithm}
\caption{Representation Learning for Bi-Linear Bandits}
\label{alg:bandit-track}
\begin{algorithmic}[1]
\State Input: arm set $\mathcal{X}$, time horizon $T$, exploration length $T_1$, rank $r$ of $\Theta^*$, spectral bound $\omega_r$ of $\Theta^*$, sampling distribution for stage 1: $D$; parameters for LowOFUL in stage $2: B, B_{\perp}, \lambda, \lambda_{\perp}$.
\State Stage 1: Explore the Low-Rank Subspace for each task $m$
\State Pull $\bx_t, \bz_t \in \X,\Z$ according to distribution $D$ and observe reward $Y_t$, for $t=1, \ldots, T_1$.
% \State Let $\widehat{\Theta}=U \widehat{S} V^T$ be the SVD of $\widehat{\Theta}$. Take the first $r$ columns of $U$ as $\widehat{U}$, the first $r$ rows of $V$ as $\widehat{V}$. Let $\widehat{U}_{\perp}$ and $\widehat{V}_{\perp}$ be orthonormal bases of the complementary subspaces of $\hat{U}$ and $\widehat{V}$.
\State Compute $\wB_1\wLambda_m\wB_2^\top \leftarrow \underset{\bB_1 \in \mathbb{R}^{d_1\times k_1},\Lambda_m\in \mathbb{R}^{k_1\times k_2}, \bB_2 \in \mathbb{R}^{d_2\times k_2}, }{\argmin }  \sum_{t=1}^{T_1}\left(Y_{t} - \bx_{t}^{\top} \bB_1 \Lambda_m \bB_2^\top\bz_{t}\right)^2$.
\State Let $\wTheta = \wB_1\wLambda_m\wB_2^\top$.
% \State Solve $\wTheta$ using the problem below:
% \begin{align*}
% \wTheta=\argmin_{\Theta \in \mathbb{R}^{d_1 \times d_2}} \frac{1}{2 T_1} \sum_{t=1}^{T_1}\left(Y_t-\bx_t^\top \wB_1\wLambda_m\wB_2^\top \bz_t\right)^2+\lambda_{T_1}\|\Theta\|_{\mathrm{nuc}} .
% \end{align*}
% \State Compute $\widehat{\bh} \leftarrow \underset{\bh \in \mathbb{R}^{k}}{\argmin }  \sum_{t=1}^{T_1}\left[\wLambda_m\wB_1^\top\bz_{t} - r_{n, t}\right]^2$
\State G-optimal design on left arms such that
\begin{align*}
\lambda^x_t = \underset{\boldsymbol{\lambda} \in \triangle_{\X}}{\argmin} \max _{\bx, \bx^{\prime} \in \hat{\X}_m}\left\|\wB_1^{\top}\left(\bx-\bx^{\prime}\right)\right\|_{\bA(\boldsymbol{\lambda}, \wB_1)^{-1}}^2
\end{align*}
\State G-optimal design on right arms such that
\begin{align*}
\lambda^z_t = \underset{\boldsymbol{\lambda} \in \triangle_{\Z}}{\argmin} \max _{\bx, \bx^{\prime} \in \hat{\X}_m}\left\|\wB_2^{\top}\left(\bz-\bz^{\prime}\right)\right\|_{\bA(\boldsymbol{\lambda}, \wB_2)^{-1}}^2
\end{align*}
\end{algorithmic}
\end{algorithm}

==> app_algo.tex <==







\begin{algorithm}
\caption{G-Optimal Design for Bilinear Bandits (\gob)}
\label{alg:bandit-pure}
\begin{algorithmic}[1]
\State Input: arm set $\X,\Z$, time horizon $n$, exploration length $n_1$, rank $r$ of $\bTheta_*$, spectral bound $S_r$ of $\bTheta_*$, sampling distribution for stage 1: $D$; parameters for stage $2: S, S_\ell^{\perp} =  \frac{8d_1 d_2 r}{\tau^E_{\ell} S^2_{r}} \log \left(\frac{d_1+d_2}{\delta_\ell}\right), \lambda, \lambda_\ell^{\perp} = \tau^G_{\ell-1}/8(d_1+d_2)r\log(1+\frac{\tau^G_{\ell-1}}{\lambda})$. Let $p=d_1d_2$, $k=(d_1+d_2)r$.
%
\State Let $\ucW_1 \leftarrow \ucW, \ell \leftarrow 1$, $\tau^G_0 = \log (4\ell^2|\X| / \delta)$.
\State Define 
% $\bA^\ell_{\bb_x} \!\!=\!\! \sum_{\bx\in\X_\ell}\bb_x\bx\bx^\top + \bLambda_\ell$, 
$\bLambda_\ell \coloneqq \mathbf{diag}[\underbrace{\lambda,\ldots,\lambda}_{k},\underbrace{\lambda_\ell^\perp,\ldots,\lambda_\ell^\perp}_{p-k}]$, $B^\ell_* \coloneqq \left(8\sqrt{\lambda S^2 +\lambda_\ell^{\perp} S^{(2),\perp}_{\ell}}\right)$ 
\State Define a vectorized arm $\ow = \left[\bx_{1: d_1}; \bz_{1: d_2}\right]$ and $\ow\in\ocW$. Let $\tau^E_{\ell} = \frac{\sqrt{8d_1 d_2 r\log (4\ell^2|\W| / \delta_\ell)}}{S_{r}}$. Let the $E$-optimal design be
\begin{align}
    \bb^E_\ell = \argmin_{\bb \in \triangle_{\ocW}}\big\|\big(\sum_{\ow\in\ocW} \bb_{\ow}\ow \ \ow^\top\big)^{-1}\big\| \label{eq:E-opt-single}
\end{align}
%
\While{$\left|\ucW_{\ell}\right|>1$}
%
\State $\epsilon_{\ell}=2^{-\ell}$
%
% \State Let $\wb_{\ell,x} = \argmax_{\bb} \log\frac{|\bA^\ell_{\bb_x}|}{|\bLambda|}$ as the solution to $D$-optimal design for $\overline{\bX}_\ell$.
% Similarly get $\wb_{\ell,z} = \argmax_{\bb} \log\frac{|\bA^\ell_{\bb_z}|}{|\bLambda|}$ as the solution to $D$-optimal design for $\Z$.
%
% \State $\epsilon_{\ell}=2^{-\ell}$, 
% $\tau^E_{\ell} = \frac{8B^\ell_*\rho^E_*\log (4\ell^2|\W| / \delta)}{\epsilon_\ell^2}$. 
% Similarly define $\tau_{\ell_z} = \frac{8k\log(1+\frac{\tau_{\ell_z-1}}{\lambda})\log (4\ell^2|\Z| / \delta)}{\epsilon^2}\left(\sqrt{56 R^2 } + \sqrt{\lambda S^2 +\lambda_{\perp} S^2_{\perp}}\right)$
%
\State \textbf{(Stage 1:) Explore the Low-Rank Subspace}
\State Pull arm $\ow \in \ocW$ exactly $\left\lceil\wb^E_{\ell, \ow} \tau^E_{\ell}\right\rceil$ times
% Pull $\bx_t \in \overline{\X}$ according to $\lceil\wb_{\ell_x}\tau_{\ell_x}\rceil$ 
% and $\lceil\wb_{\ell_z}\tau_{\ell_z}\rceil$ respectively 
and observe rewards $r_t$, for $t=1, \ldots, \tau^E_{\ell}$.
\State Compute $\wTheta_{\ell}$ using \eqref{eq:convex-prog}.
% $=\arg \min _{\bTheta \in \mathbb{R}^{d_1 \times d_2}} L_{n_1}(\bTheta)+\lambda_{n_1}\|\bTheta\|_{\mathrm{nuc}}, \quad L_{n_1}(\bTheta)=\langle\bTheta, \bTheta\rangle-\frac{2}{n_1} \sum_{i=1}^{n_1}\left\langle\tilde{\psi}_\nu\left(y_i \cdot S\left(X_i\right)\right), \bTheta\right\rangle $.
%
\State \textbf{(Stage 2:) Reduction to low dimensional linear bandits}  
\State Let the SVD of $\wTheta_{\ell} = \wU_\ell\wD_{\ell}\wV_{\ell}^\top$. Then rotate the arm sets following \eqref{eq:rotated-arm-set-phase} to build $\ucW$.
%
% : $\X^{\prime}_\ell=\left\{\left[\wU \wU_{\perp}\right]^{\top} \bx: \bx \in \X\right\}$ and $\Z^{\prime}_\ell=\left\{\left[\wV \wV_{\perp}\right]^{\top} \bz: \bz \in \Z\right\}$.
% Define a vectorized arm set so that the last $\left(d_1-r\right) \cdot\left(d_2-r\right)$ components are from the complementary subspaces:
% \begin{align*}
% \X_\ell=\left\{\left[\vec\left(\bx_{1: r} \bz_{1: r}^{\top}\right) ; \vec\left(\bx_{r+1: d_1} \bz_{1: r}^{\top}\right) ; \vec\left(\bx_{1: r} \bz_{r+1: d_2}^{\top}\right) ; \vec\left(\bx_{r+1: d_1} \bz_{r+1: d_2}^{\top}\right)\right] \in \mathbb{R}^{d_1 d_2}: \bx \in \X^{\prime}, \bz \in \Z^{\prime}\right\} .
% \end{align*}
% %
%
\State Let $\wb^G_{\ell} = \argmin_{\bb_{\uw}}\max_{\uw,\uw'\in\ucW_\ell} \|\uw-\uw'\|^2_{(\sum_{\uw\in\ucW} \bb_{\uw}\uw\ \uw^\top + \bLambda_\ell/n )^{-1}}$. 
%
\State Define $\rho^G(\Y(\ucW_{\ell})) = \min_{\bb_{\uw}}\max_{\uw,\uw'\in\ucW_\ell} \|\uw-\uw'\|^2_{(\sum_{\uw\in\ucW} \bb_{\uw}\uw\ \uw^\top + \bLambda_\ell/n )^{-1}}$. 
%
\State Set 
$\tau^G_{\ell} \!\!=\!\! \frac{8(B^\ell_*)^2\rho^G(\Y(\W_\ell))\log (4\ell^2|\W| / \delta)}{\epsilon_\ell^2}$. 
%
%
Then pull arm $\uw \in \ucW$ exactly $\left\lceil\wb_{\ell, \uw} \tau^G_{\ell}\right\rceil$ times and \indent construct the least squares estimator $\wtheta_{\ell}$ using only the observations of this phase where $\wtheta_\ell$ \indent is defined in \eqref{eq:least-sq-reg}. Note that $\wtheta_\ell$ is also rotated following \eqref{eq:rotated-arm-set-phase}.
% =\argmin_{\btheta} \frac{1}{2}\|\uW_\ell \btheta-\br\|_2^2+\frac{1}{2}\|\btheta\|_{\bLambda_\ell}^2$
\State Eliminate arms such that 
%\begin{align*}
$\ucW_{\ell+1} \leftarrow \ucW_{\ell} \backslash\left\{\uw \in \ucW_{\ell}: \max_{\uw^{\prime} \in \ucW_{\ell}}\left\langle \uw^{\prime}-\uw, \wtheta_{\ell}\right\rangle>2 \epsilon_{\ell}\right\}$
% \end{align*}
\State $\ell \leftarrow \ell+1$
\EndWhile
\State Output the arm in $\ucW_{\ell}$ and reshape to get the $\widehat{\bx}_*$ and $\widehat{\bz}_*$
\end{algorithmic}
\end{algorithm}

==> backup.tex <==
\begin{lemma}\textbf{(Theorem 16 from \citet{lu2021low})}
\label{lemma:Theta-est}
Sample $X_1, \ldots, X_n \in \mathbb{R}^{d_1 \times d_2}$ from $\X$ according to $D$. Then under \Cref{assm:dist-D}, any optimal solution to the nuclear norm optimization problem \eqref{eq:convex-prog} using $\lambda_n \asymp \frac{1}{n \min \left\{d_1, d_2\right\}} \log \left(\frac{n}{\delta}\right) \log \left(\frac{d_1+d_2}{\delta}\right)$ satisfies:
\begin{align*}
\left\|\wTheta-\bTheta^*\right\|_F^2 \asymp \frac{\left(d_1+d_2\right)^3 r}{n}
\end{align*}
with probability $1-\delta$.
The goal of stage 1 is to estimate the row/column subspaces of $\bTheta^*$, below the corollary that characterizes their convergence.
\end{lemma}

The goal of stage 1 is to estimate the row/column subspaces of $\bTheta^*$, below the corollary that characterizes their convergence.

\begin{corollary}
\textbf{Restatement of Corollary 17 of \citet{lu2021low} (adapted from Jun et al. (2019))}. Suppose we compute $\wTheta$ by solving the convex problem in \eqref{eq:convex-prog} as an estimate of the matrix $\bTheta^*$. After stage 1 of ESTR with $n_1=\Omega\left(r\left(d_1+d_2\right)\right)$ satisfying the condition of \Cref{lemma:Theta-est}, we have, with probability at least $1-\delta$,
\begin{align*}
\left\|\widehat{U}_{\perp}^T U^*\right\|_F\left\|\widehat{V}_{\perp}^T V^*\right\|_F \leq \frac{\left\|\bTheta^*-\wTheta\right\|_F^2}{\omega_r^2} \leq C \frac{\lambda_{n_1}^2 r}{\alpha_1^2 \omega_r^2}:=\gamma\left(n_1\right) \asymp \frac{\left(d_1+d_2\right)^3 r}{n_1 \omega_r^2},
\end{align*}
where $\omega_r>0$ denotes the lower bound of the $r$-th singular value of $\bTheta^*$ and $C$ represents some constant.
\end{corollary}


Once we have the above result we can do the following:

\textbf{1.} Let $\wTheta=U \widehat{S} V^T$ be the SVD of $\wTheta$. Take the first $r$ columns of $U$ as $\widehat{U}$, the first $r$ rows of $V$ as $\widehat{V}$. Let $\widehat{U}_{\perp}$ and $\widehat{V}_{\perp}$ be orthonormal bases of the complementary subspaces of $\widehat{U}$ and $\widehat{V}$.

\textbf{2.} Refine Standard Linear Bandit Algorithm. 
Rotate the arm feature set: $\X^{\prime}:=\left\{\left[\begin{array}{ll}\hat{U} & \hat{U}_{\perp}\end{array}\right]^T X\left[\widehat{V} \widehat{V}_{\perp}\right]: X \in \X\right\}$
Define a vectorized arm feature set so that the last $\left(d_1-r\right)\left(d_2-r\right)$ components are from the complementary subspaces:
\begin{align*}
\X_{\text {vec }}^{\prime}:=\left\{\operatorname{vec}\left(X_{1: r, 1: r}^{\prime}\right) ; \operatorname{vec}\left(X_{r+1: d_1, 1: r}^{\prime}\right) ; \operatorname{vec}\left(X_{1: r, r+1: d_2}^{\prime}\right) ; \operatorname{vec}\left(X_{r+1: d_1, r+1: d_2}^{\prime}\right): X^{\prime} \in \X^{\prime}\right\}
\end{align*}

\textbf{3
.} Run G-optimal design in $\X_{\text {vec }}^{\prime}$ which has a low dimension of $k=\left(d_1+d_2\right) r-r^2$. 

\subsection{Regret Bound for Single Task \gob}

\begin{definition}\textbf{(Restricted Strong Convexity (RSC) (Wainwright, 2019))}. For a given norm $\|\cdot\|$, regularizer $\Phi(\cdot)$, and $X_1, \ldots, X_n \in \mathbb{R}^{d_1 \times d_2}$, the matrix $\widehat{\Gamma}=\frac{1}{n} \widetilde{X}^T \widetilde{X}$, where $\tilde{x}_i:=\operatorname{vec}\left(X_i\right)$ and $\widetilde{X}:=\left[\tilde{x}_1^T ; \ldots ; \tilde{x}_n^T\right]$, satisfies a restricted strong convexity (RSC) condition with curvature $\kappa>0$ and tolerance $\tau_n^2$ if
\begin{align*}
\widetilde{\Delta}^T \widehat{\Gamma} \widetilde{\Delta}=\frac{1}{n} \sum_{t=1}^n\left\langle X_t, \Delta\right\rangle^2 \geq \kappa\|\Delta\|^2-\tau_n^2 \Phi^2(\Delta)
\end{align*}
for all $\Delta \in \mathbb{R}^{d_1 \times d_2}$, and we denote $\operatorname{vec}(\Delta)$ by $\widetilde{\Delta}$.
\end{definition}

\begin{definition}\textbf{(Cone set)}
Define $\mathbb{K}(s):=\mathbb{B}_{\text {rank }}(s) \cap \mathbb{B}_F(1)$ and the cone set $\mathbb{C}(s):=\left\{v:\|v\|_{\text {nuc }} \leq \sqrt{s}\|v\|_F\right\}$, all matrices defined in these sets are in $\mathbb{R}^{d_1 \times d_2}$.
\end{definition}

We prove the following theorem about distribution $D$ (see Assumption 2). We first state a support lemma below.

\begin{lemma}\textbf{(Restatement of Lemma 22 (RSC condition))}
Suppose $s \geq 1$ and $\widehat{\Gamma}$ is an estimator of $\Sigma$ satisfying the deviation condition $(\tilde{v}:=\operatorname{vec}(v))$
\begin{align*}
\left|\tilde{v}^T(\widehat{\Gamma}-\Sigma) \tilde{v}\right| \leq \frac{\lambda_{\min }(\Sigma)}{54}, \forall v \in \mathbb{K}(2 s),
\end{align*}
where $\mathbb{K}(2 s)$ is defined in Definition 3. Then we have the RSC condition
\begin{align*}
\tilde{v}^T \widehat{\Gamma} \tilde{v} \geq \frac{\lambda_{\min }(\Sigma)}{2}\|v\|_F^2-\frac{\lambda_{\min }(\Sigma)}{2 s}\|v\|_{n u c}^2
\end{align*}
\end{lemma} 

\begin{lemma}\textbf{(Restatement of Theorem 15 from \citet{lu2021low}
 (Distribution $D$ satisfies RSC))}. Sample $X_1, \ldots, X_n \in \mathbb{R}^{d_1 \times d_2}$ from $\X$ according to $D$, and define $\tilde{x}_i:=\operatorname{vec}\left(X_i\right), \widetilde{X}=\left[\tilde{x}_1^T ; \ldots ; \tilde{x}_n^T\right] \in \mathbb{R}^{n \times d_1 d_2}$ and $\widehat{\Gamma}:=\frac{1}{n} \tilde{X}^T \tilde{X}$. Then under Assumption 2, there exists constants $c_1, c_2>0$, such that with probability $1-\delta$,
\begin{align*}
\widetilde{\Theta}^T \widehat{\Gamma} \widetilde{\Theta}=\frac{1}{n} \sum_{i=1}^n\left\langle X_i, \Theta\right\rangle^2 \geq \frac{c_1}{d_1 d_2}\|\Theta\|_F^2-\frac{c_2\left(d_1+d_2\right)}{n d_1 d_2}\|\Theta\|_{n u c}^2, \forall \Theta \in \mathbb{R}^{d_1 \times d_2}
\end{align*}
for $n=\Omega\left(\left(d_1+d_2\right) \log \left(\frac{1}{\delta}\right)\right)$, where $\widetilde{\Theta}:=\operatorname{vec}(\Theta)$.
\end{lemma}

Lemma 3 states that sampling $X$ from $\X$ according to distribution $D$ guarantees that the sampled arms satisfies RSC condition. We further show that under RSC condition, the estimated $\wTheta$ is guaranteed to converge to $\bTheta$ at a fast rate in Lemma 1.


\begin{proof}
Using the results in Lemma 2, together with the substitutions
\begin{align*}
\widehat{\Gamma}-\Sigma=\frac{1}{n} \widetilde{X}^T \tilde{X}-\Sigma, \text { and } s:=\frac{1}{c} \frac{n}{d_1+d_2} \min \left\{\frac{\lambda_{\min }^2(\Sigma)}{\sigma^4}, 1\right\}
\end{align*}
where $n \geq c\left(d_1+d_2\right) / \min \left\{\frac{\lambda_{m i n}^2(\Sigma)}{\sigma^4}, 1\right\}$ so $s \geq 1$, we see that it suffices to show that
\begin{align*}
D(s):=\sup _{v \in \mathbb{K}(2 s)}\left|\tilde{v}^T(\widehat{\Gamma}-\Sigma) \tilde{v}\right| \leq \frac{\lambda_{\min }(\Sigma)}{54}
\end{align*}
with high probability.
Note that by modified Lemma 15 ( in Appendix $G$ ) in Loh and Wainwright (2011), we simply change the 1 /3-covering set for sparsity vectors to the $1 / 3$-covering set for $\mathbb{K}(2 s)$, whose covering number is $27^{2 s\left(d_1+d_2+1\right)}$ by Lemma 7 , and achieve
\begin{align*}
\Pb(D(s) \geq t) \leq 2 \exp \left(-c^{\prime} n \min \left(\frac{t^2}{\sigma^4}, \frac{t}{\sigma^2}\right)+2 s\left(d_1+d_2+1\right) \log 27\right),
\end{align*}
for some univeral constant $c^{\prime}>0$. Setting $t=\frac{\lambda_{\min }(\Sigma)}{54}$, we see that there exists some $c_2>0$, such that
\begin{align*}
\Pb\left(D(s) \geq \frac{\lambda_{\min }(\Sigma)}{54}\right) \leq 2 \exp \left(-c_2 n \min \left(\frac{\lambda_{\min }^2(\Sigma)}{\sigma^4}, 1\right)\right),
\end{align*}
which establishes the result.
Set $\delta$ equals to the right side of last inequality, one can get the desired gurantee for $n$ in Theorem 15 .
\end{proof}


\subsubsection{Proof of Lemma 1}

We first state the support lemma below.

\begin{lemma}\textbf{(Restatement of Lemma 23 from (Converence under RSC, adapted from Proposition 10.1 in Wainwright (2019)))}
Suppose the observations $X_1, \ldots, X_n$ satisfies the non-scaled RSC condition in Definition [2, such that
\begin{align*}
\frac{1}{n_1} \sum_{t=1}^n\left\langle X_t, \Theta\right\rangle^2 \geq \kappa\|\Theta\|_F^2-\tau_n^2\|\Theta\|_{n u c}^2, \forall \Theta \in \mathbb{R}^{d_1 \times d_2}
\end{align*}
Then under the event $G:=\left\{\left\|\frac{1}{n} \sum_{t=1}^n \eta_t X_t\right\|_{o p} \leq \frac{\lambda_n}{2}\right\}$, any optimal solution $\wtheta$ to Equation 6 satisfies the bound below:
\begin{align*}
\left\|\wtheta-\bTheta^*\right\|_F^2 \leq 4.5 \frac{\lambda_n^2}{\kappa^2} r
\end{align*}
where $r=\operatorname{rank}\left(\bTheta^*\right)$ and $\frac{1}{\tau_n^2} \geq \frac{64 r}{\kappa}$.
\end{lemma}



\begin{proof}
According to Lemma 3, there exists constants $c_1$ and $c_2$ such that with probability at least $1-\delta$, we have below RSC condition
\begin{align*}
\frac{1}{n} \sum_{t=1}^n\left\langle X_t, \Theta\right\rangle^2 \geq \frac{c_1}{d_1 d_2}\|\Theta\|_F^2-\frac{c_2\left(d_1+d_2\right)}{n d_1 d_2}\|\Theta\|_{n u c}^2, \forall \Theta \in \mathbb{R}^{d_1 \times d_2}
\end{align*}
Lemma 4 can be applied under above RSC condition, then under event $G\left(\lambda_n\right):=\left\{\left\|\frac{1}{n} \sum_{t=1}^n \eta_t X_t\right\|_{o p} \leq \frac{\lambda_n}{2}\right\}$, we can easily conclude the theorem. Thus, it remains to figure out $\lambda_n$ such that event $G\left(\lambda_n\right)$ can hold with high probability.

Define the rare event $E:=\left\{\max _{t=1, \ldots, n_1}\left|\eta_t\right|>\sqrt{2 \log \left(\frac{4 n_1}{\delta}\right)}\right\}$, so that $\Pb(E) \leq \delta / 2$ can be proved by the definition of sub-Gaussian. By matrix Bernstein inequality, the probability of $G\left(\lambda_n\right)^c$ can be bounded by:
\begin{align*}
\begin{aligned}
P\left(\left\|\frac{1}{n} \sum_{t=1}^n \eta_t X_t\right\|_{o p}>\varepsilon\right) & \leq P\left(\left\|\frac{1}{n} \sum_{t=1}^n \eta_t X_t\right\|_{o p}>\varepsilon \mid E^c\right)+P(E) \\
& \leq\left(d_1+d_2\right) \exp \left(\frac{-n \varepsilon^2 / 2}{2 \log \left(\frac{4 n}{\delta}\right) \max \left\{1 / d_1, 1 / d_2\right\}+\varepsilon \sqrt{2 \log \left(\frac{4 n}{\delta}\right) / 3}}\right)+\delta / 2,
\end{aligned}
\end{align*}
where the last inequality is by matrix Bernstein using the fact that
\begin{align*}
\max \left\{\left\|\sum_{t=1}^n \mathbb{E} \eta_t^2 X_t X_t^T\right\|_{o p},\left\|\sum_{t=1}^n \mathbb{E} \eta_t^2 X_t^T X_t\right\|_{o p}\right\} \leq 2 n \log \left(\frac{4 n}{\delta}\right) \max \left\{1 / d_1, 1 / d_2\right\} .
\end{align*}
For $\left(d_1+d_2\right) \exp \left(\frac{-n \varepsilon^2 / 2}{2 \log \left(\frac{4 n}{b}\right) \max \left\{1 / d_1, 1 / d_2\right\}+\varepsilon \sqrt{2 \log \left(\frac{4 n}{b}\right) / 3}}\right) \leq \delta / 2$ to hold, we need
\begin{align*}
\epsilon^2=\frac{C^{\prime}}{n \min \left\{d_1, d_2\right\}} \log \left(\frac{n}{\delta}\right) \log \left(\frac{d_1+d_2}{\delta}\right)
\end{align*}
holds for some constant $C^{\prime}$. Take $\lambda_n=2 \varepsilon$, we need $\lambda_n^2=\frac{C}{n \min \left\{d_1, d_2\right\}} \log \left(\frac{n}{\delta}\right) \log \left(\frac{d_1+d_2}{\delta}\right)$ and under this condition we have $P\left(G\left(\lambda_n\right)\right) \geq 1-\delta$. We complete the proof by noting that the scaling of the right hand side in Lemma 23 under above choice of $\lambda_n$ is indeed $\frac{\left(d_1+d_2\right)^3 r}{n}$.
 \end{proof}

==> g_optimal_bi.tex <==
We first state the optimal design for the Bi-linear Bandits in this section in \Cref{alg:bandit-track}. 


\begin{algorithm}
\caption{Optimal Design for Bilinear Bandits (\gob)}
\label{alg:bandit-track}
\begin{algorithmic}[1]
\State Input: arm set $\X,\Z$, time horizon $n$, exploration length $n_1$, rank $r$ of $\bTheta^*$, spectral bound $S_r$ of $\bTheta^*$, sampling distribution for stage 1: $D$; parameters for stage $2: S, S_{\perp}, \lambda, \lambda_{\perp}$.
\State (Stage 1:) Explore the Low-Rank Subspace for each task $m$
\State Pull $\bx_t, \bz_t \in \X,\Z$ according to distribution $D$ and observe reward $Y_t$, for $t=1, \ldots, T_1$.
% \State Let $\wTheta=U \widehat{S} V^T$ be the SVD of $\wTheta$. Take the first $r$ columns of $U$ as $\widehat{U}$, the first $r$ rows of $V$ as $\widehat{V}$. Let $\widehat{U}_{\perp}$ and $\widehat{V}_{\perp}$ be orthonormal bases of the complementary subspaces of $\hat{U}$ and $\widehat{V}$.
\State Compute $\wTheta_{n_1}=\arg \min _{\bTheta \in \mathbb{R}^{d_1 \times d_2}} L_{n_1}(\bTheta)+\lambda_{n_1}\|\bTheta\|_{\mathrm{nuc}}, \quad L_{n_1}(\bTheta)=\langle\bTheta, \bTheta\rangle-\frac{2}{n_1} \sum_{i=1}^{n_1}\left\langle\tilde{\psi}_\nu\left(y_i \cdot S\left(X_i\right)\right), \bTheta\right\rangle $.
% \State Let $\wTheta = \wB_1\wLambda_m\wB_2^\top$.
\State (Stage 2:) Rotate the arm sets: $\X^{\prime}=\left\{\left[\widehat{\bU} \widehat{\bU}_{\perp}\right]^{\top} \bx: \bx \in \X\right\}$ and $\mathcal{Z}^{\prime}=\left\{\left[\widehat{\bV} \widehat{\bV}_{\perp}\right]^{\top} \mathrm{z}: \mathrm{z} \in \mathcal{Z}\right\}$.
Define a vectorized arm set so that the last $\left(d_1-r\right) \cdot\left(d_2-r\right)$ components are from the complementary subspaces:
\begin{align*}
\X=\left\{\left[\operatorname{vec}\left(\bx_{1: r} \mathrm{z}_{1: r}^{\top}\right) ; \operatorname{vec}\left(\bx_{r+1: d_1} \mathrm{z}_{1: r}^{\top}\right) ; \operatorname{vec}\left(\bx_{1: r} \mathrm{z}_{r+1: d_2}^{\top}\right) ; \operatorname{vec}\left(\bx_{r+1: d_1} \mathrm{z}_{r+1: d_2}^{\top}\right)\right] \in \mathbb{R}^{d_1 d_2}: \bx \in \X^{\prime}, \mathrm{z} \in \mathcal{Z}^{\prime}\right\} .
\end{align*}
%
\State Let $\X_1 \leftarrow \X, \ell \leftarrow 1$.
\State Define $\bA^\ell_{\bb} = \sum_{\bx\in\X_\ell}\bb_x\bx\bx^\top + \bLambda$, and $\bLambda = \mathrm{diag}[\underbrace{\lambda,\ldots,\lambda}_{k},\underbrace{\lambda_\perp,\ldots,\lambda_\perp}_{p-k}]$ 
\While{$\left|\X_{\ell}\right|>1$}
\State Let $\wb_{\ell} = \argmax_{\bb} \log\frac{|\bA^\ell_{\bb}|}{|\bLambda|}$ as the solution to $D$-optimal design.  
%
\State $\epsilon_{\ell}=2^{-\ell}$, %$\tau_{\ell}=2 d \epsilon_{\ell}^{-2} \log \left(4 \ell^2|\X| / \delta\right)$, 
$\tau_{\ell} = \frac{k\log(1+\frac{n}{\lambda})\log (4\ell^2|\X| / \delta)}{\epsilon^2}\left(\sqrt{56 R^2 } + \sqrt{\lambda S^2 +\lambda_{\perp} S^2_{\perp}}\right)$
%
\State Pull arm $x \in \X$ exactly $\left\lceil\wb_{\ell, x} \tau_{\ell}\right\rceil$ times and construct the least squares estimator $\wtheta_{\ell}$ using \indent only the observations of this round where $\wtheta_\ell=\arg \min_{\btheta} \frac{1}{2}\|\bX_\ell \btheta-\mathbf{y}\|_2^2+\frac{1}{2}\|\btheta\|_{\boldsymbol{\bLambda}}^2$
\State Eliminate arms such that 
%\begin{align*}
$\X_{\ell+1} \leftarrow \X_{\ell} \backslash\left\{x \in \X_{\ell}: \max _{x^{\prime} \in \X_{\ell}}\left\langle \bx^{\prime}-\bx, \wtheta_{\ell}\right\rangle>2 \epsilon_{\ell}\right\}$
% \end{align*}
\State $\ell \leftarrow \ell+1$
\EndWhile
\State Output: $\X_{\ell}$


% \State Solve $\wTheta$ using the problem below:
% \begin{align*}
% \wTheta=\argmin_{\bTheta \in \mathbb{R}^{d_1 \times d_2}} \frac{1}{2 T_1} \sum_{t=1}^{T_1}\left(Y_t-\bx_t^\top \wB_1\wLambda_m\wB_2^\top \bz_t\right)^2+\lambda_{T_1}\|\bTheta\|_{\mathrm{nuc}} .
% \end{align*}
% \State Compute $\widehat{\bh} \leftarrow \underset{\bh \in \mathbb{R}^{k}}{\argmin }  \sum_{t=1}^{T_1}\left[\wLambda_m\wB_1^\top\bz_{t} - r_{n, t}\right]^2$
% \State G-optimal design on left arms such that
% \begin{align*}
% \lambda^x_t = \underset{\boldsymbol{\lambda} \in \triangle_{\X}}{\argmin} \max _{\bx, \bx^{\prime} \in \hat{\X}_m}\left\|\wB_1^{\top}\left(\bx-\bx^{\prime}\right)\right\|_{\bA(\boldsymbol{\lambda}, \wB_1)^{-1}}^2
% \end{align*}
% \State G-optimal design on right arms such that
% \begin{align*}
% \lambda^z_t = \underset{\boldsymbol{\lambda} \in \triangle_{\Z}}{\argmin} \max _{\bx, \bx^{\prime} \in \hat{\X}_m}\left\|\wB_2^{\top}\left(\bz-\bz^{\prime}\right)\right\|_{\bA(\boldsymbol{\lambda}, \wB_2)^{-1}}^2
% \end{align*}
\end{algorithmic}
\end{algorithm}



% Note that both \citet{kang2022efficient, lu2021low} do not use any optimal designs and their regret is problem independent that scales with $O(\sqrt{(d_1 + d_2)r T})$. When we use the G-optimal design we intend to get a problem-dependent bound.

% To see this, first, consider the simple bi-linear bandit setting when you observe both the left and right arms $\bx_t$ and $\bz_t$. Then the reward is given by
% \begin{align*}
%     r_t = \bx_t^\top\bTheta_*\bz_t + \eta_t = \langle \bTheta_*, \bx_t\bz_t^\top \rangle + \eta_t &= \vec(\bTheta_*)^\top\vec(\bX_t) + \eta_t \\
%     %%%%%%%%%%%%%%%
%     &=  \vec(\bTheta_*)^\top\vec(\bX_t) + \eta_t = (\bTheta^v_*)^\top\bX^v_t + \eta_t
% \end{align*}
% where $\bX_t$ is a rank one $d_1\times d_2$ matrix. So $\bX^v_t,\bTheta^v_*$ are vectors in $\R^{d_1 d_2}$. Then we can show that
% \begin{align*}
%     \wTheta^v_n = \left((\bX^v_n)^\top(\bX^v_n)\right)^{-1}(\bX^v_n)^\top\bY_n
% \end{align*}
% Since $\eta_t\sim \SG(0,\sigma^2\bI)$, then it follows then that for any $Z^v_t\in\R^{d_1 d_2}$ we have that
% \begin{align*}
%     (\bZ^v_t)^\top\left(\wTheta^v_n - \bTheta_*\right) \sim \SG\left(0, (\bZ^v_t)^\top \left((\bX^v_n)^\top(\bX^v_n)\right)^{-1}\bZ^v_t\right)
% \end{align*}
% This results in a G-optimal design that scales with $d_1d_2$. Applying RAGE \citep{fiez2019sequential} algorithm on this feature vector $\bX^v_t$ will result in a regret that scales with $O\left(\sqrt{d_1d_2 T}\right)$. 


% To overcome this, with the additional knowledge that $\bTheta_*$ has rank $r$ we can do somewhat better. 
Let
$\wTheta_{n_1}$ be an estimate $\bTheta_*$. We can get the estimate by solving the problem below:
\begin{align}
\wTheta=\arg \min _{\bTheta \in \mathbb{R}^{d_1 \times d_2}} L_{n_1}(\bTheta)+\lambda_{n_1}\|\bTheta\|_{\mathrm{nuc}}, \quad L_{n_1}(\bTheta)=\langle\bTheta, \bTheta\rangle-\frac{2}{n_1} \sum_{i=1}^{n_1}\left\langle\tilde{\psi}_\nu\left(y_i \cdot S\left(X_i\right)\right), \bTheta\right\rangle \label{eq:convex-prog}
\end{align}

% \begin{align}
% \wTheta_{n_1}=\argmin_{\bTheta \in \mathbb{R}^{d_1 \times d_2}} \frac{1}{2 n_1} \sum_{t=1}^{n_1}\left(Y_t- \bx_t^\top \bTheta\bz_t\right)^2+\lambda_{n_1}\|\bTheta\|_{\text {nuc }} \label{eq:convex-prog}
% \end{align}


We first state the assumption to sample according to the distribution $D$ in the first stage.
%
\begin{assumption}
\label{assm:dist-D}
There exists a sampling distribution $D$ over $\X,\Z$ with covariance matrix $\Sigma$, such that $\lambda_{\min }(\Sigma) \asymp \frac{1}{d_1 d_2}$ and $D$ is sub-Gaussian with parameter $\sigma^2 \asymp \frac{1}{d_1 d_2}$. 
\end{assumption}


 











\subsection{Main Regret Bound Proof}

\textbf{Stage 1:} We run \gob\ in stage 1 with $n_1  \asymp \sqrt{d_1 d_2 r n \log \left(\left(d_1+d_2\right) / \delta\right)} / S_{r}$. 
%
% We can guarantee $\left\|\wTheta-\bTheta^*\right\|_F^2 \asymp \frac{\left(d_1+d_2\right)^3 r}{n_1}$. We get the estimated row/column subspaces of $\bTheta^*$ simply by running an SVD step.
We have the following result from \citet{kang2022efficient}.

\begin{theorem}
\label{theorem:kang-low-rank}
\textbf{(Restatement of Theorem 4.1 in \citet{kang2022efficient})} For any low-rank linear model with samples $X_1 \ldots, X_{n_1}$ drawn from $\X$ according to $\mathcal{D}$ then for the optimal solution to the nuclear norm regularization problem in \eqref{eq:convex-prog} with $\nu=\sqrt{2 \log \left(2\left(d_1+d_2\right) / \delta\right) /\left(\left(4 \sigma_0^2+S_0^2\right) M n_1 d_1 d_2\right)}$ and
\begin{align*}
\lambda_{n_1}=4 \sqrt{\frac{2\left(4 \sigma_0^2+S_0^2\right) M d_1 d_2 \log \left(2\left(d_1+d_2\right) / \delta\right)}{n_1}},
\end{align*}
with probability at least $1-\delta$ it holds that:
\begin{align*}
\left\|\wTheta- \mu^*\bTheta^*\right\|_F^2 \leq \frac{C_1 d_1 d_2 r \log \left(\frac{2\left(d_1+d_2\right)}{\delta}\right)}{n_1},
\end{align*}
for $C_1=36\left(4 \sigma_0^2+S_0^2\right) M$, $\|X\|_F,\left\|\bTheta^*\right\|_F \leq S_0$, some nonzero constant $\mu^*$, and $\mathbb{E}\left[\left(S^{\mathrm{P}}(X)\right)_{i j}^2\right] \leq M, \forall i, j$.
\end{theorem}

% \textbf{Stage 2:} Rotate the arm feature set: 
% $$
% \X^{\prime}:=\left\{\left[\begin{array}{ll}\hat{U} & \hat{U}_{\perp}\end{array}\right]^T X\left[\widehat{V} \widehat{V}_{\perp}\right]: X \in \X\right\}.
% $$
% Define a vectorized arm feature set so that the last $\left(d_1-r\right)\left(d_2-r\right)$ components are from the complementary subspaces:
% \begin{align*}
% \X_{\text {vec }}^{\prime}:=\left\{\operatorname{vec}\left(X_{1: r, 1: r}^{\prime}\right) ; \operatorname{vec}\left(X_{r+1: d_1, 1: r}^{\prime}\right) ; \operatorname{vec}\left(X_{1: r, r+1: d_2}^{\prime}\right) ; \operatorname{vec}\left(X_{r+1: d_1, r+1: d_2}^{\prime}\right): X^{\prime} \in \X^{\prime}\right\}
% \end{align*}
% %
% Then run G-optimal design in $\X_{\text {vec }}^{\prime}$ which has a low dimension of $k=\left(d_1+d_2\right) r-r^2$. 


\subsubsection{Stage 2 Proof}



\textbf{Reduction to linear bandits:}   Recall that $\bTheta^*= \bU^* \mathbf{S}^* \bV^{*^{\top}}$ is the SVD of $\bTheta^*$ (where $\mathbf{S}^*$ is $r \times r$ diagonal) and that $\widehat{\bU}_{\perp}$ and $\widehat{\bV}_{\perp}$ are the complementary subspace of $\widehat{\bU}$ and $\widehat{\bV}$ respectively. Let $\mathbf{H}=\left[\widehat{\bU} \widehat{\bU}_{\perp}\right]^{\top} \bTheta^*\left[\widehat{\bV} \widehat{\bV}_{\perp}\right]$ be a rotated version of $\bTheta^*$. Then we have
\begin{align*}
\bTheta^* & =\left[\widehat{\bU} \widehat{\bU}_{\perp}\right] \mathbf{H}\left[\widehat{\bV} \widehat{\bV}_{\perp}\right]^{\top} \quad \text { and } \\
\bx^{\top} \bTheta^* \mathbf{z} & =\left(\left[\widehat{\bU} \widehat{\bU}_{\perp}\right]^{\top} \bx\right)^{\top} \mathbf{H}\left(\left[\widehat{\bV} \widehat{\bV}_{\perp}\right]^{\top} \mathbf{z}\right) .
\end{align*}

Thus, the bilinear bandit problem with the unknown $\bTheta^*$ with arm sets $\X$ and $\mathcal{Z}$ is equivalent to the one with the unknown $\mathbf{H}$ with arm sets 
$$
\X^{\prime}=\left\{\bx^{\prime}=\left[\widehat{\bU} \widehat{\bU}_\perp\right]^{\top} \bx \mid \bx \in \X\right\}
$$ and 
$$
\mathcal{Z}^{\prime}= \left\{\bz^{\prime}=\left[\widehat{\bV} \widehat{\bV}_{\perp}\right]^{\top} \mathbf{z} \mid \bz \in \mathcal{Z}\right\}
$$
As mentioned earlier, this problem can be cast as a $d_1 d_2$-dimensional linear bandit problem by considering the unknown vector $\btheta^*=\operatorname{vec}(\mathbf{H})$. The difference is, however, that we have learned something about the subspace in stage 1. We define $\btheta^*$ to be a rearranged version of vec $(\mathbf{H})$ so that the last $\left(d_1-r\right) \cdot\left(d_2-r\right)$ dimensions of $\btheta^*$ are $M_{i j}$ for $i \in\left\{r+1, \ldots, d_1\right\}$ and $j \in\left\{r+1, \ldots, d_2\right\}$; that is, letting $k:=d_1 d_2-\left(d_1-r\right) \cdot\left(d_2-r\right)$,
\begin{align*}
& \btheta_{1: k}^*=\left[\operatorname{vec}\left(\mathbf{H}_{1: r, 1: r}\right) ; \operatorname{vec}\left(\mathbf{H}_{r+1: d_1, 1: r}\right) ; \operatorname{vec}\left(\mathbf{H}_{1: r, r+1: d_2}\right)\right] \\
& \btheta_{k+1: p}^*=\operatorname{vec}\left(\mathbf{H}_{r+1: d_1, r+1: d_2}\right) .
\end{align*}
Then we have
\begin{align*}
\left\|\btheta_{k+1: p}^*\right\|_2^2 & =\sum_{i>r \wedge j>r} H_{i j}^2=\left\|\widehat{\mathbf{U}}_{\perp}^{\top}\left(\mathbf{U}^* \mathbf{S}^* \bV^{* \top}\right) \widehat{\bV}_{\perp}\right\|_F^2 \\
& \leq\left\|\widehat{\mathbf{U}}_{\perp}^{\top} \mathbf{U}^*\right\|_F^2\left\|\mathbf{S}^*\right\|_2^2\left\|\widehat{\bV}_{\perp}^{\top} \bV^*\right\|_F^2  \leq \frac{d_1 d_2 r}{n_1 S_{r}^2} \log \left(\frac{d_1+d_2}{\delta}\right):=S_{\perp},
\end{align*}
which implies $\left\|\btheta_{k+1: p}^{\star}\right\|_2=\mathcal{O}\left(d_1d_2 r / n_1\right)$ by \Cref{theorem:kang-low-rank}. 




\subsubsection{Properties of each phase in Second Stage}

Let us denote the vector $\bx\in\R^p$ a vectorized form of $\X^\prime,\Z^\prime$ where $p=d_1d_2$. So $\bx=[\bx^\prime;\bz^\prime]$.
%
% First, recall that we use $\bX$ and $\bZ$ to denote the reduced arm set $\bX^\prime$ and $\bZ^\prime$ in stage $2$.
%
Let the length of the $\ell$-th phase be $\tau$. 
Let at the $\ell$-th phase the actions sampled be denoted by the matrix $\bX_\ell\in\R^{\tau\times p}$ and $\bx\in\bX_\ell$. Define the positive diagonal matrix $\bLambda$. Specifically, we define $\bLambda= \operatorname{diag}\left(\lambda, \ldots, \lambda, \lambda_{\perp}, \ldots, \lambda_{\perp}\right)$, where $\lambda$ occupies the first $k$ diagonal entries and $\lambda_{\perp}$ the last $p-k$ positions. 
%
Then the estimation of $\btheta_*$ be
\begin{align*}
\wtheta_\ell=\arg \min_{\btheta} \frac{1}{2}\|\bX_\ell \btheta-\mathbf{y}\|_2^2+\frac{1}{2}\|\btheta\|_{\boldsymbol{\bLambda}}^2=\left(\bLambda+\bX_\ell^{\top} \bX_\ell\right)^{-1} \bX_\ell^{\top} \bY_\ell .
\end{align*}

The following lemma follows from Lemma 7 of \citet{valko2014spectral}. 
\begin{lemma}
\label{eq:conc-lemma-bilin}
For any fixed $\bx \in \R^{p}$ and any $\delta>0$, we have that if $\beta\left(\btheta_*, \delta\right)=2 R \sqrt{14 \log (2 / \delta)}+\left\|\btheta_*\right\|_{\bLambda}$, then at time $t_{\ell}$ (beginning of phase $\ell$):
\begin{align*}
\Pb\left(\left|\bx^{\top}\left(\wtheta_\ell-\btheta_*\right)\right| \leq\|\bx\|_{\bV_\ell^{-1}} \beta\left(\btheta_*, \delta\right)\right) \geq 1-\delta
\end{align*}
where, $\bV_{\ell} \coloneqq \sum_{s=\ell_{j}-1}^{\ell_j}\bx_s\bx_s^\top +  \bLambda$.
\end{lemma}

\begin{proof}
Defining $\bxi_\ell=\sum_{s=t_{\ell-1}+1}^{t_{\ell}} \bx_s \eta_s$, we have:
\begin{align}
\left|\bx^{\top}\left(\wtheta_\ell-\btheta_*\right)\right| & \overset{(a)}{=}\left|\bx^{\top}\left(-\bV_\ell^{-1} \bLambda \btheta_*+\bV_\ell^{-1} \bxi_\ell\right)\right| \nonumber\\
& \overset{(b)}{\leq}\left|\bx^{\top} \bV_\ell^{-1} \bLambda \btheta_*\right|+\left|\bx^{\top} \bV_\ell^{-1} \bxi_\ell\right| \label{eq:triangle-ineq}
\end{align}
where, $(a)$ follows from Woodbury matrix identity and rearranging the terms, and $(b)$ follows from the triangle inequality. 
% To see $(a)$ observe that ($\eta$ is the noise vector)
% \begin{align*}
%     \bx^{\top}\left(\wtheta_\ell-\btheta_*\right) &= \bx^{\top}\left(\left(\bLambda+\bX_\ell^{\top} \bX_\ell\right)^{-1} \bX_\ell^{\top} \bY_\ell - \btheta_*\right) = \bx^{\top}\left(\left(\bLambda+\bX_\ell^{\top} \bX_\ell\right)^{-1} \bX_\ell^{\top} \left(\bX_\ell\btheta_* + \eta\right) - \btheta_*\right)\\
%     %%%%%%%%%%%%%%%%%
%     &= \bx^{\top}\left(\left(\left(\bX_\ell^{\top} \bX_\ell\right)^{-1} - \left(\bX_\ell^{\top} \bX_\ell\right)^{-1}\left(\bLambda+\bX_\ell^{\top} \bX_\ell\right)^{-1}\right) \bX_\ell^{\top} \left(\bX_\ell\btheta_* + \eta\right) - \btheta_*\right)\\
%     %%%%%%%%%%%%%%%%%
%     &= \bx^{\top}\left(\left(\btheta_* - \left(\bX_\ell^{\top} \bX_\ell\right)^{-1}\left(\bLambda+\bX_\ell^{\top} \bX_\ell\right)^{-1}\right) \bX_\ell^{\top} \left(\bX_\ell\btheta_* + \eta\right) - \btheta_*\right)
% \end{align*}


The first term in the right-hand side of \eqref{eq:triangle-ineq} is bounded as:
\begin{align*}
\left|\bx^{\top} \bV_\ell^{-1} \bLambda \btheta_*\right| & \leq\left\|\bx^\top \bV_\ell^{-1} \bLambda^{1 / 2}\right\|\left\|\bLambda^{1 / 2} \btheta_*\right\| \\
%%%%%%%%%%%%%%%%%
& \overset{(a)}{=}\left\|\btheta_*\right\|_{\bLambda} \sqrt{\bx^{\top} \bV_\ell^{-1} \bLambda \bV_j^{-1} \bx} \\
& \leq\left\|\btheta_*\right\|_{\bLambda} \sqrt{\bx^{\top} \bV_\ell^{-1} \bx}=\left\|\btheta_*\right\|_{\bLambda}\|\bx\|_{\bV_{\ell}^{-1}}
\end{align*}
where, $(a)$ follows as $\|\btheta_*\|_\bLambda = \sqrt{\btheta_*^\top\bLambda\btheta_*} = \|\bLambda^{1/2}\btheta_*\|$ and similarly for $\left\|\bx^\top \bV_\ell^{-1} \bLambda^{1 / 2}\right\|$. 
%
Now consider the second term in the r.h.s. of \eqref{eq:triangle-ineq}. We have:
\begin{align*}
\left|\bx^{\top} \bV_\ell^{-1} \bxi_\ell\right|=\left|\sum_{s=t_{\ell-1}+1}^{t_{\ell}}\left(\bx^{\top} \bV_\ell^{-1} \bx_s\right) \eta_s\right|
\end{align*}
Let us notice that the points $\left(\bx_s\right)$ selected by the algorithm during phase $\ell-1$ only depend on the proportion $\lambda^*$ (the G-optimal design) and do not
% their width $\|\bx\|_{\bV_s^{-1}}$ which does not 
depend on the rewards received during the phase $\ell-1$. Thus, given $\mathcal{F}_{j-2}$, the sequence $\left(\bx_s\right)_{t_{\ell-1}+1 \leq s<t_{\ell}}$ is deterministic. Consequently, one may use a variant of Azuma's inequality (\citet{shamir2011variant}):
\begin{align*}
& \Pb\left(\left|\bx^{\top} \bV_\ell^{-1} \bxi_\ell\right|^2 \leq 28 R^2 2 \log (2 / \delta) \times \bx^{\top} \bV_\ell^{-1}\left(\sum_{s=t_{\ell-1}+1}^{t_{\ell}} \bx_s \bx_s^{\top}\right) \bV_\ell^{-1} \bx \mid \mathcal{F}_{\ell-2}\right) \geq 1-\delta,
\end{align*}
from which we deduce:
\begin{align*}
& \Pb\left(\left|\bx^{\top} \bV_\ell^{-1} \bxi_\ell\right|^2 \leq 56 R^2 \bx^{\top} \bV_\ell^{-1} \bx \log (2 / \delta) \mid \mathcal{F}_{\ell-2}\right) \geq 1-\delta,
\end{align*}
since $\sum_{s=t_{\ell-1}+1}^{t_{\ell}} \bx_s \bx_s^{\top} \prec \bV_\ell$. Thus: 
\begin{align*}
& \qquad \Pb\left(\left|\bx^{\top} \bV_\ell^{-1} \bxi_\ell\right| \leq 2 R\|\bx\|_{\bV_\ell^{-1}} \sqrt{14 \log (2 / \delta)}\right) \geq 1-\delta
\end{align*}
Combining everything we get that 
\begin{align*}
\Pb\left(\left|\bx^{\top}\left(\wtheta_\ell-\btheta_*\right)\right| \leq2 R \sqrt{14 \log (2 / \delta)}+\left\|\btheta_*\right\|_{\bLambda}\right)\leq 1-\delta.
\end{align*}
\end{proof}

We need the following support lemma from \citet{valko2014spectral}. 

% These are as follows:
% \begin{lemma}\textbf{(Restatement of Lemma 11 from \citet{valko2014spectral})} For any real positive-definite matrix $\bA$ with only simple eigenvalue multiplicities and any vector $\bx$ such that $\|\bx\|_2 \leq 1$ we have that the determinant $\left|\mathbf{A}+\bx\bx^{\top}\right|$ is maximized by a vector $\bx$ which is aligned with an eigenvector of $\mathbf{A}$.
% \end{lemma}

\begin{lemma}\textbf{(Restatement of Lemma 4 from \citet{valko2014spectral})}
\label{lemma:valko-lemma-4}
Let $\bLambda=\operatorname{diag}\left(\lambda_1, \ldots, \lambda_p\right)$ be any diagonal matrix with strictly positive entries. Then for any vectors $\left(\bx_s\right)_{1 \leq s \leq t}$, such that $\left\|\bx_s\right\|_2 \leq 1$ for all $1 \leq s \leq t$, we have that the determinant $\left|\mathbf{V}_t\right|$ of $\mathbf{V}_t=\bLambda+\sum_{s=1}^t \bx_s \bx_s^{\top}$ is maximized when all $\bx_s$ are aligned with the axes.
\end{lemma}


\begin{lemma}
\label{lemma:valko-lemma-effective-dim}
Let $k$ be the effective dimension. Then
\begin{align*}
\log \frac{\left|\mathbf{V}_t\right|}{|\bLambda|} \leq 2 k \log \left(1+\frac{n}{\lambda}\right)
\end{align*}
when $\lambda_{\perp}=\frac{n}{k \log \left(1+n / \lambda\right)}$ and $t\leq n$.
\end{lemma}

\begin{proof}
We want to bound the determinant $\left|\mathbf{V}_t\right|$ under the coordinate constraints $\left\|\bx_t\right\|_2 \leq 1$. Let:
\begin{align*}
M\left(\bx_1, \ldots, \bx_t\right)=\left|\bLambda+\sum_{s=1}^t \bx_s \bx_s^{\top}\right|
\end{align*}
%
From \Cref{lemma:valko-lemma-4} we deduce that the maximum of $M$ is reached when all $\bx_t$ are aligned with the axes. Let the number of samples of these axes-aligned $\bx_s$'s be denoted as  $t_1,t_2,\ldots,t_p$ such that $\sum_{i=1}^p t_i = t$.  
%
Then we can show that
\begin{align*}
& M=\max _{\bx_1, \ldots, \bx_t ; \bx_t \in\left\{\mathrm{e}_1, \ldots, \mathbf{e}_p\right\}}\left|\bLambda+\sum_{s=1}^t \bx_s \bx_s^{\top}\right| \\
%%%%%%%%%%%%%%%%%%
& =\max_{t_1, \ldots, t_p,\text { positive integers, } \sum_{i=1}^p t_i=t}\left|\operatorname{diag}\left(\lambda_i+t_i\right)\right| \\
%%%%%%%%%%%%%%%%%%
& \leq \quad \max_{t_1, \ldots, t_p,\text { positive integers, } \sum_{i=1}^p t_i=t} \prod_{i=1}^p\left(\lambda_i+t_i\right)
\end{align*}
%
Now we can show that
\begin{align*}
\log \frac{\left|\mathbf{V}_t\right|}{|\bLambda|} & \leq \sum_{i=1}^k \log \left(1+\frac{t}{\lambda}\right)+\sum_{i=k+1}^p \log \left(1+\frac{t_i}{\lambda_i}\right) \\
%%%%%%%%%%%%%%%%%
& \leq k \log \left(1+\frac{t}{\lambda}\right)+\sum_{i=1}^p \frac{t_i}{\lambda_{\perp}} \\
%%%%%%%%%%%%%%%%%
& \leq k \log \left(1+\frac{t}{\lambda}\right)+\frac{t}{\lambda_{\perp}} \\
%%%%%%%%%%%%%%%%%
& \overset{(a)}{\leq} 2 k \log \left(1+\frac{n}{\lambda}\right) 
\end{align*}
where, $(a)$ follows for $\lambda_{\perp} = \frac{n}{k \log \left(1+n / \lambda\right)}$
\end{proof}

Next, we can use \citet{jamieson2022interactive} Frank-Wolfe algorithm (in section 2.3.1) with the 
$$
g(\bb) = \log \frac{\left|\sum_{i}\bb_i\bx_i\bx_i^\top + \bLambda\right|}{|\bLambda|} = \log \left|\sum_{i}\bb_i\bx_i\bx_i^\top + \bLambda\right|-\log|\bLambda|,
$$ 
setting $I_k=\argmax _{i}\left\|\bx_i\right\|_{\left(\sum_{j=1}^A \bb_j^k \bx_j \bx_j^{\top} + \bLambda\right)^{-1}}^2$, 
and stopping condition $\max _i\left\|\bx_i\right\|_{\left(\sum_{j=1}^A \bb_j^{k+1} \bx_j \bx_j^{\top} +\bLambda \right)^{-1}}^2 \leq 2 k\log(1+\frac{n}{\lambda})$. 
%
It follows then that for any $\bb \in \triangle_{\X}$ we have by Kiefer-Wolfowitz that $[\nabla g(\lambda)]_{\bx^{\prime}}=\left\|\bx^{\prime}\right\|_{\left(\sum_{\bx \in \X} \bb_x \bx \bx^{\top} + \bLambda\right)^{-1}}^2 \geq 2k\log(1 + \frac{n}{\lambda})$.
This is because $\bLambda$ does not depend on $\bx$. 
%
Rest of the proof follows by the same way as in section 2.3.1 in \citet{jamieson2022interactive}. 
%
This will result in a support size of $\bb$ at most $k\log(1+\frac{n}{\lambda})(k\log(1+\frac{n}{\lambda}) + 1)/2$.
%
Hence, it follows that maximizing the $\log \frac{\left|\mathbf{V}_t\right|}{|\bLambda|}$ function will result in a support of $|\bb^*|\leq \frac{k\log(1+\frac{n}{\lambda})(k\log(1+\frac{n}{\lambda}) + 1)}{2}$.

\begin{proposition}
If $\lambda^*_\ell$ is the $D$-optimal design for $\X_\ell$ then if we pull arm $\bx \in \X_\ell$ exactly $\left\lceil\tau \bb_{\ell^*}\right\rceil$ times for some $\tau>0$ and compute the least squares estimator $\wtheta_\ell$. Then for each $\bx \in \X_\ell$ we have with probability at least $1-\delta$
\begin{align*}
    \Pb\bigg(\bigcup_{\bx \in \X_\ell}\bigg\{\left|\left\langle \bx, \wtheta_\ell-\btheta^*\right\rangle\right|&\leq B^*\sqrt{\dfrac{k\log(1+\frac{n}{\lambda}) \log \left(2|\X| / \delta\right)}{\tau}} \bigg\}\bigg) \geq 1-\delta.
\end{align*}
where, we have $\left\|\btheta^*\right\|_{\Lambda} \leq \sqrt{\lambda\left\|\btheta_{1: k}\right\|_2^2+\lambda_{\perp}\left\|\btheta_{k+1: p}\right\|_2^2} \leq \sqrt{\lambda} S+\sqrt{\lambda_{\perp}} S_{\perp}$ and $B^*=\sqrt{56 R^2 } + \sqrt{\lambda S^2 +\lambda_{\perp} S^2_{\perp}}$.
\end{proposition}

\begin{proof}
% First, recall from \citet{lattimore2020bandit} Kiefer-Wolfowitz Theorem 21.1 that $G-$ and $D-$ optimal design are equivalent. Formulating the above G-optimal design problem into a D-optimal design, we have
% \begin{align*}
%     ff
% \end{align*}
From Woodbury Matrix Identity we know that $(\bA+\bB)^{-1}=\bA^{-1}-\left(\bA+\bA \bB^{-1} \bA\right)^{-1}$. It follows then that 
\begin{align*}
    \bx^\top(\bA+\bB)^{-1}\bx = \bx^\top\left(\bA^{-1}-\left(\bA+\bA \bB^{-1} \bA\right)^{-1}\right)\bx \leq \bx^\top\bA^{-1}\bx = \|\bx\|_{\bA^{-1}}. 
\end{align*}
Hence we can show that,
\begin{align}
    &\|\bx\|_{\left(\sum_{\bx \in \X_\ell}\lceil\tau \bb_{\ell^*}\rceil \bx \bx^{\top} + \bLambda\right)^{-1}} 
    % = \bx^\top\left(\sum_{\bx \in \X_\ell}\lceil\tau \bb_{\ell^*}\rceil \bx \bx^{\top} + \bLambda \right)^{-1}\bx\\
    % %%%%%%%%%%%%%%%%%%
    % &=\bx^\top\left(\left(\sum_{\bx \in \X_\ell}\lceil\tau \bb_{\ell^*}\rceil \bx \bx^{\top}\right)^{-1} -  \left(\sum_{\bx \in \X_\ell}\lceil\tau \bb_{\ell^*}\rceil \bx \bx^{\top}\right)^{-1}\left(\sum_{\bx \in \X_\ell}\lceil\tau \bb_{\ell^*}\rceil \bx \bx^{\top}+ \sum_{\bx \in \X_\ell}\lceil\tau \bb_{\ell^*}\rceil \bx \bx^{\top}\bLambda^{-1}\sum_{\bx \in \X_\ell}\lceil\tau \bb_{\ell^*}\rceil \bx \bx^{\top} \right)\right)\bx \\
    % %%%%%%%%%%%%%%%%%%%%
    \leq \bx^\top\left(\sum_{\bx \in \X_\ell}\lceil\tau \bb_{\ell^*}\rceil \bx \bx^{\top}\right)^{-1}\bx \label{eq:matrix-inv}
\end{align}


Further the support of $\lambda^*$ is less than $\frac{k\log(1+\frac{n}{\lambda})(k\log(1+\frac{n}{\lambda})+1)}{2} \leq (k\log(1+\frac{n}{\lambda}))^2$. Also note that $\left\|\btheta^*\right\|_{\Lambda} \leq \sqrt{\lambda\left\|\btheta_{1: k}\right\|_2^2+\lambda_{\perp}\left\|\btheta_{k+1: p}\right\|_2^2} \leq \sqrt{\lambda} S+\sqrt{\lambda_{\perp}} S_{\perp}$.
%
Then we can show that
\begin{align*}
\left\langle \bx, \wtheta_\ell -\btheta^*\right\rangle & \leq\|\bx\|_{\left(\sum_{\bx \in \X_\ell}\lceil\tau \bb_{\ell^*}\rceil \bx \bx^{\top} + \bLambda\right)^{-1}} \left(2R\sqrt{14 \log (2 / \delta)} + \sqrt{\lambda} S+\sqrt{\lambda_{\perp}} S_{\perp} \right) \\
%%%%%%%%%%%%%%%%%%%
& \leq \frac{1}{\sqrt{\tau}}\|\bx\|_{\left(\sum_{\bx \in \X_\ell} \bb_{\ell^*} \bx \bx^{\top}\right)^{-1}} \left(2R\sqrt{14 \log (2 / \delta)} + \sqrt{\lambda} S+\sqrt{\lambda_{\perp}} S_{\perp}\right)\\
%%%%%%%%%%%%%%%%%%%
& \leq \sqrt{\frac{56 R^2 k\log(1+\frac{n}{\lambda}) \log (2 / \delta)}{\tau}} + \sqrt{\dfrac{k\log(1+\frac{n}{\lambda})(\lambda S^2 +\lambda_{\perp} S^2_{\perp})\log(2/\delta)}{\tau}}\\
%%%%%%%%%%%%%%%%%%%%%
&= \sqrt{\frac{k\log(1+\frac{n}{\lambda})\log (2 / \delta)}{\tau}}\left(\underbrace{\sqrt{56 R^2 } + \sqrt{\lambda S^2 +\lambda_{\perp} S^2_{\perp}}}_{B^*}\right)
\end{align*}
and we have taken at most $\tau+\frac{k\log(1+\frac{n}{\lambda})(k\log(1+\frac{n}{\lambda})+1)}{2}$ pulls. Thus, for any $\delta \in(0,1)$ we have 
\begin{align*}
\Pb\bigg(\bigcup_{\bx \in \X_\ell}\bigg\{\left|\left\langle \bx, \wtheta_\ell-\btheta^*\right\rangle\right|&\geq B^*\sqrt{\dfrac{ k\log(1+\frac{n}{\lambda}) \log \left(2|\X| / \delta\right)}{\tau}} \bigg\}\bigg) \leq \delta.
\end{align*}
\end{proof}



% We assume the $\bx\in\X_{\text {vec }}^{\prime}$ in this stage where $\bx\in\R^k$ and $k=\left(d_1+d_2\right) r-r^2$. We assume that $\X_{\ell}$ is the active set in phase $\ell$. 

\begin{lemma}
Assume that $\max_{\bx \in \X}\left\langle \bx^{\star}-\bx, \btheta^*\right\rangle \leq 4$. With probability at least $1-\delta$, we have $\bx^{\star} \in \X_{\ell}$ and $\max _{\bx \in \X_{\ell}}\left\langle \bx^{\star}-\bx, \btheta^*\right\rangle \leq 8 \epsilon_{\ell}$ for all 
$\ell \in \mathbb{N}$.
\end{lemma}

\begin{proof}
For any $\mathcal{V} \subseteq \X$ and $\bx \in \mathcal{V}$ define the event
\begin{align*}
\mathcal{E}_{\bx, \ell}(\mathcal{V})=\left\{\left|\left\langle \bx, \wtheta_{\ell}(\mathcal{V})-\btheta^*\right\rangle\right| \leq \epsilon_{\ell}\right\}
\end{align*}
where it is implicit that $\wtheta_{\ell}:=\wtheta_{\ell}(\mathcal{V})$ is the $G$-optimal design constructed in the algorithm at stage $\ell$ with respect to $\X_{\ell}=\mathcal{V}$. Note that this is precisely the analogous events of multi-armed bandits.
%
The key piece of the analysis is that
\begin{align*}
\begin{aligned}
\Pb\left(\bigcup_{\ell=1}^{\infty} \bigcup_{\bx \in \X_{\ell}}\left\{\mathcal{E}_{\bx, \ell}^c\left(\X_{\ell}\right)\right\}\right) & \leq \sum_{\ell=1}^{\infty} \Pb\left(\bigcup_{\bx \in \X_{\ell}}\left\{\mathcal{E}_{\bx, \ell}^c\left(\X_{\ell}\right)\right\}\right) \\
& =\sum_{\ell=1}^{\infty} \sum_{\mathcal{V} \subseteq \X} \Pb\left(\bigcup_{\bx \in \mathcal{V}}\left\{\mathcal{E}_{\bx, \ell}^c(\mathcal{V})\right\}, \X_{\ell}=\mathcal{V}\right) \\
& =\sum_{\ell=1}^{\infty} \sum_{\mathcal{V} \subseteq \X} \Pb\left(\bigcup_{\bx \in \mathcal{V}}\left\{\mathcal{E}_{\bx, \ell}^c(\mathcal{V})\right\}\right) \Pb\left(\X_{\ell}=\mathcal{V}\right) \\
& \leq \sum_{\ell=1}^{\infty} \sum_{\mathcal{V} \subseteq \X} \frac{\delta|\mathcal{V}|}{2 \ell^2|\X|} \Pb\left(\X_{\ell}=\mathcal{V}\right) \leq \delta
\end{aligned}
\end{align*}
Thus, in what follows, assume $\mathcal{E}:=\bigcap_{\bx \in \X} \bigcap_{\ell=1}^{\infty}\left\{\mathcal{E}_{\bx, \ell}\left(\X_{\ell}\right)\right\}$ holds.
Fix any $\ell$ for which $\bx^{\star} \in \X_{\ell}$ (note $\bx^{\star} \in \X_1$ ). Then for any $\bx \in \X_{\ell}$ we have
\begin{align*}
\begin{aligned}
\left\langle \bx-\bx^{\star}, \wtheta_{\ell}\right\rangle & =\left\langle \bx, \wtheta_{\ell}-\btheta^*\right\rangle-\left\langle \bx^{\star}, \wtheta_{\ell}-\btheta^*\right\rangle+\left\langle \bx-\bx^{\star}, \btheta^*\right\rangle \\
& \leq 2 \epsilon_{\ell}
\end{aligned}
\end{align*}
which implies $\bx^{\star} \in \X_{\ell+1}$. Thus, $\bx^{\star} \in \X_{\ell}$ for all $\ell$. On the other hand, any $\bx$ for which $\left\langle \bx^{\star}-\bx, \btheta^*\right\rangle>$ $4 \epsilon_{\ell}$ we have
\begin{align*}
\begin{aligned}
\max _{\bx^{\prime} \in \X_{\ell}}\left\langle \bx^{\prime}-\bx, \wtheta_{\ell}\right\rangle & \geq\left\langle \bx^{\star}-\bx, \wtheta_{\ell}\right\rangle \\
& =\left\langle \bx^{\star}, \wtheta_{\ell}-\btheta^*\right\rangle-\left\langle \bx, \wtheta_{\ell}-\btheta^*\right\rangle+\left\langle \bx^{\star}-\bx, \btheta^*\right\rangle \\
& >2 \epsilon_{\ell}
\end{aligned}
\end{align*}
which implies $\max _{\bx \in \X_{\ell+1}}\left\langle \bx, \btheta^*\right\rangle \geq\left\langle \bx^{\star}, \btheta^*\right\rangle-4 \epsilon_{\ell}=\left\langle \bx^{\star}, \btheta^*\right\rangle-8 \epsilon_{\ell+1}$.
\end{proof}

\subsubsection{Regret Bound for G-optimal design in Second Stage}

\begin{theorem} 
    Let The $S$ and $S_{\perp}$ are valid upper bounds of $\left\|\btheta^*\right\|_2$ and $\left\|\btheta_{k+1: p}^*\right\|_2$, respectively, with high probability. Let $S_{\perp}=  \frac{d_1 d_2 r}{n_1 S_{r}^2} \log \left(\frac{d_1+d_2}{\delta}\right)$.
    %
Substituting all the values in $B^* = \sqrt{56 R^2 } + \sqrt{\lambda S^2 +\lambda_{\perp} S^2_{\perp}}$ like above we get the total regret of $R_{n_2} \leq \widetilde{O}\left(\sqrt{k n }\right)$ where $\widetilde{O}$ hides logarithmic factors.
%
\end{theorem}

Due to the subspace estimation error in the first phase the error in the second phase suffers an additional factor 
\begin{align*}
    n_2 S_{\perp} \leq  n \frac{d_1 d_2 r}{n_1 S_{r}^2} \log \left(\frac{d_1+d_2}{\delta}\right)
\end{align*}
where $S_\perp =  \frac{d_1 d_2 r}{n_1 S_{r}^2} \log \left(\frac{d_1+d_2}{\delta}\right)$.
%
% $S_2 \gamma\left(n_1\right)$
% \begin{align*}
%     \quad\left\|\bTheta^*\right\|_2 \leq S_2, \quad
%     %%
% \gamma\left(n_1\right)&=\frac{\left\|\mathbf{X}^{-1}\right\|_2^2\left\|\mathbf{Z}^{-1}\right\|_2^2}{\left(S_r\right)^2} \cdot C_1^2\left(\frac{S_2}{S_r}\right)^4 \sigma^2 \cdot \frac{(d_1+d_2)^3 r}{n_1}
% \end{align*}

We assume that $\X_{\ell}$ is the active set in phase $\ell$. 
%
For any $\ell \geq\left\lceil\log _2\left(8 \Delta^{-1}\right)\right\rceil$ we have that $\X_{\ell}=\left\{\bx^{\star}\right\}$. Suppose you run for $n_2$ timesteps. Then for any $\nu \geq 0$ the regret is bounded by:
\begin{align*}
& \sum_{\bx \in \X \backslash \bx^{\star}} \Delta_x T_x=\sum_{\bx \in \X \backslash \bx^{\star}: \Delta_x \leq \nu} \Delta_x T_x+\sum_{\bx \in \X \backslash \bx^{\star}: \Delta_x>\nu} \Delta_x T_x \\
%%%%%%%%%%%%%%%%%%%%
& \leq \nu n_2 +\sum_{\ell=1}^{\infty} \sum_{\bx \in \X_{\ell} \backslash \bx^{\star}: \Delta_x>\nu} \Delta_x\left\lceil\tau_{\ell} \wb_{\ell, \bx}\right\rceil \\
%%%%%%%%%%%%%%%%%%%%
& \leq n_2 \nu+\sum_{\ell=1}^{\lceil\log _2\left(8(\Delta \vee \nu)^{-1}\right)\rceil} 8 \epsilon_{\ell}\left(\left|\operatorname{support}\left(\wb_{\ell}\right)\right|+\tau_{\ell}\right) \\
%%%%%%%%%%%%%%%%%%%%
& =n_2 \nu+\hspace*{-2em}\sum_{\ell=1}^{\lceil\log _2\left(8(\Delta \vee \nu)^{-1}\right)\rceil} \hspace*{-2em} 8 \epsilon_{\ell}\left(\frac{(k\log(1+\frac{n}{\lambda})+1) k\log(1+\frac{n}{\lambda})}{2}  +  2 k\log(1+\frac{n}{\lambda})\log(1+\frac{n}{\lambda}) \epsilon_{\ell}^{-2} B^*\log \left(4 \ell^2|\X| / \delta\right)\right) %\\
\end{align*}
\begin{align*}
%%%%%%%%%%%%%%%%%%%%%
& \leq n_2 \nu+4(k\log(1+\frac{n}{\lambda})+1) k\log(1+\frac{n}{\lambda})\left\lceil\log _2\left(8(\Delta \vee \nu)^{-1}\right)\right\rceil \\
%%%%%
&\quad + \sum_{\ell=1}^{\left\lceil\log _2\left(8(\Delta \vee \nu)^{-1}\right)\right\rceil} 16 k\log(1+\frac{n}{\lambda}) \epsilon_{\ell}^{-1} B^*\log \left(4 \ell^2|\X| / \delta\right) \\
%%%%%%%%%%%%%%%%%%%%%%
& \leq n_2 \nu+4(k\log(1+\frac{n}{\lambda})+1) k\log(1+\frac{n}{\lambda})\left\lceil\log _2\left(8(\Delta \vee \nu)^{-1}\right)\right\rceil\\
%%%%%%%%
&\quad +16 k\log(1+\frac{n}{\lambda}) B^* \log \left(4 \log _2^2\left(16(\Delta \vee \nu)^{-1}\right)|\X| / \delta\right) \sum_{\ell=1}^{\lceil\log _2\left(8(\Delta \vee \nu)^{-1}\right)\rceil} 2^{\ell} \\
%%%%%%%%%%%%%%%%%%%%%%%
& \leq n_2 \nu+4(k\log(1+\frac{n}{\lambda})+1) k\log(1+\frac{n}{\lambda})\left\lceil\log _2\left(8(\Delta \vee \nu)^{-1}\right)\right\rceil\\
%%%%%%%%
&\quad +512 k\log(1+\frac{n}{\lambda})(\Delta \vee \nu)^{-1} B^*\log \left(4 \log _2^2\left(16(\Delta \vee \nu)^{-1}\right)|\X| / \delta\right)
\end{align*}
% Setting $\nu=0$ yields a regret bound of $O\left(k \Delta^{-1} \log \left(|\X| \log \left(\Delta^{-1}\right) / \delta\right)\right)$ which implies $R_{n_2} \leq c \frac{k}{\Delta} \log (|\X| T)$. 
Minimizing over $\nu>0$ yields a regret bound of 
$$
R_{n_2} \leq O\left(\sqrt{k\log(1+\frac{n}{\lambda}) T (B^*)^2 \log \left(\log \left(\frac{n}{ k\log(1+\frac{n}{\lambda})} \right)  |\X| / \delta\right)}\right)
$$ 
which implies $R_{n_2} \leq c \sqrt{k n (B^*)^2\log(1+\frac{n}{\lambda})\log (|\X| n)}$.
%

We denote by $s_i^*$ the $i$-th largest singular value of $\bTheta^*$. Recall that we assume that the rank $r$ of the matrix is known and that $s_r^* \geq S_r$ for some known $S_r>0$. 
%
Finally following \citet{jun2019bilinear} we set $S_{\perp}=\mathcal{O}\left(1 / n_1\right)$ to be a valid upper bound of $\left\|\bTheta_{k+1: p}^*\right\|_2$, and 
%
% By setting $n_1=\bTheta(\sqrt{T})$, the regret bound in Corollary 1 scales with $\sqrt{T}$ rather than $T$.
% Concretely, using (9), 
we set $S=S_0$, $\left\|\bTheta^*\right\|_2 \leq S_2$, and $S_{\perp}=  \frac{d_1 d_2 r}{n_1 S_{r}^2} \log \left(\frac{d_1+d_2}{\delta}\right)$. 
%
%
% $S_2 \cdot \gamma\left(n_1\right)$ where
% \begin{align*}
% \left\|\bTheta^*\right\|_F &\leq S_F, \quad\left\|\bTheta^*\right\|_2 \leq S_2\\
% %%%%%%%%%%%%%%%%%%
% \gamma\left(n_1\right)&=\frac{\left\|\mathbf{X}^{-1}\right\|_2^2\left\|\mathbf{Z}^{-1}\right\|_2^2}{\left(S_r\right)^2} \cdot C_1^2\left(\frac{S_2}{S_r}\right)^4 \sigma^2 \cdot \frac{(d_1+d_2)^3 r}{n_1} .
% \end{align*}
The $S$ and $S_{\perp}$ are valid upper bounds of $\left\|\btheta^*\right\|_2$ and $\left\|\btheta_{k+1: p}^*\right\|_2$, respectively, with high probability. 
%
% Note we must use $S_2$, $S_r$, and $S_2 / S_r$ instead of $s_1^*, s_r^*$, and $\kappa$, respectively since the latter variables are unknown to the learner. 
Substituting all the values in $B^* = \sqrt{56 R^2 } + \sqrt{\lambda S^2 +\lambda_{\perp} S^2_{\perp}}$ like above we get the total regret of $R_{n_2} \leq \widetilde{O}\left(\sqrt{k n }\right)$ where $\widetilde{O}$ hides logarithmic factors.


\subsubsection{Combining Stage 1 and Stage 2}

\begin{theorem}
    The total regret combining stage 1 and 2 for \gob\ is given by
    \begin{align*}
        R_n \leq \widetilde{O}\left(\left(\frac{\sqrt{r d_1 d_2}}{S_{r}}+\sqrt{k}\right) \sqrt{n}\right)
    \end{align*}
    where we assume that the rank $r$ of the matrix is known and that $s_r^* \geq S_r$ for some known $S_r>0$. 
\end{theorem}

In this section, we combine the two stages.
%
Let us define $r_t=\max_{\bX} \left(\left\langle \bX, \bTheta^*\right\rangle\right)-\left(\left\langle \bX_t, \bTheta^*\right\rangle\right)$, the instantaneous regret at time $t$ where the matrix $\bX$ is the rank one matrix such that $\bX = \bx\bz^\top$. We can easily bound the regret for stage 1 as $\sum_{t=1}^{n_1} r_t \leq 2 S_0 n_1$. For the second stage, we have a bound as 
$$
\sum_{t=n_1+1}^n r_t \leq \widetilde{O}\left( \sqrt{kn}+ n S_{\perp}\right) \leq \widetilde{O}\left(\sqrt{kn} + n \frac{d_1 d_2 r}{n_1 S_{r}^2} \log \left(\frac{d_1+d_2}{\delta}\right)\right)
$$
Therefore, the overall regret is:
$$
\sum_{t=1}^n r_t \leq \widetilde{O}\left(2 S_0 n_1+ \sqrt{kn} + n \frac{d_1 d_2 r}{n_1 S_{r}^2} \log \left(\frac{d_1+d_2}{\delta}\right)\right)
$$
After plugging the choice of $n_1 \asymp \sqrt{d_1 d_2 r n \log \left(\left(d_1+d_2\right) / \delta\right)} / S_{r}$ it holds that
$$
\sum_{t=1}^n r_t \leq \widetilde{O}\left(\left(\frac{\sqrt{r d_1 d_2}}{S_{r}} + \sqrt{k}\right) \sqrt{n}\right) \lesssim \widetilde{O}\left(\left(\frac{\sqrt{r d_1 d_2}}{S_{r}}+\sqrt{k}\right) \sqrt{n}\right)=\widetilde{O}\left(\left(d_1+d_2\right) r \sqrt{n}\right)
$$
This concludes the regret-bound proof.





==> noisy_feature.tex <==
\section{Noisy Feature}

We first consider the linear bandit setting. 
\begin{assumption}\textbf{(Linear Bandit with noisy feature):} Consider the bandit 
$\operatorname{B}(\A, H, \mathrm{r})$ as a linear bandit with a feature map $\phi: \mathcal{A} \rightarrow \mathbb{R}^d$, if for any $h \in[H]$, there exist an unknown vector $\btheta_* \in \mathbb{R}^d$, such that for any $a \in \mathcal{A}$, we have
\begin{align*}
r_h(a) & =\left\langle\phi(a),\btheta_*\right\rangle + \eta_h.
\end{align*}
where, $\eta_h \sim \SG(0,\sigma^2\bI)$. We assume that the learner observes the noisy/corrupted feature
\begin{align*}
    \ophi(a) = \phi(a) + \epsilon_h(a)
\end{align*}
where $\epsilon_h(a)\sim \SG(\bf{0}_{d\times 1}, \bSigma_{*})$ and $\bSigma_*\in\R^{d\times d}$ is unknown to the learner.
\end{assumption}

A similar setting can also be studied for the representation learning setting.
\begin{assumption}\textbf{(Representation learning with Linear Bandit with noisy feature):} Consider the bandit 
$\operatorname{B}(\A, H, \mathrm{r})$ as a linear bandit with a feature map $\phi: \mathcal{A} \rightarrow \mathbb{R}^d$, if for any $h \in[H]$, there exist an unknown vector $\btheta_* \in \mathbb{R}^d$, such that for any $a \in \mathcal{A}$, we have
\begin{align*}
r_h(a) & =\left\langle\phi(a),\btheta_*\right\rangle + \eta_h.
\end{align*}
where, $\eta_h \sim \SG(0,\sigma^2\bI)$. Further, we assume that $\btheta_* = \bB \bw_*$ where $\bB\in \R^{d\times k}$ and $\bw\in\R^k$ such that $d\gg k$. We assume that the learner observes the noisy/corrupted feature
\begin{align*}
    \ophi(a) = \phi(a) + \epsilon_h(a)
\end{align*}
where $\epsilon_h(a)\sim \SG(\bf{0}_{d\times 1}, \bSigma_{*})$ and $\bSigma_*\in\R^{d\times d}$ is unknown to the learner.
\end{assumption}

This is similar to assuming the rich observation feature $\phi(a)$ admits a low dimensional feature representation $\bB^\top\phi(a) \in \R^k$. 

The key challenge in learning is twofold. First, note that we only observe the noisy feature matrix $\oX = \bX + \bE$ where $\bX\in\R^{n\times d}$ is the true feature matrix observed for $n$ rounds, and $\bE\in\R^{n\times d}$ is the noisy added to the matrix. To recover the true matrix $\bX$ we can use techniques from non-convex optimization in \citet{chen2020noisy} as follows:
We can solve the following convex program
\begin{align}
\bZ_{\mathrm{cvx}} = \underset{\bZ \in \mathbb{R}^{n \times d}}{\operatorname{minimize}} \quad  \frac{1}{2} \sum_{(i, j) \in \Omega}\left(Z_{i j}-\oX_{i j}\right)^2+\lambda\|\bZ\|_*, \label{eq:opt}
\end{align}
where $\|\bZ\|_*$ denotes the nuclear norm (i.e., the sum of singular values) of $\bZ$-a convex surrogate for the rank function. 


\begin{theorem} \textbf{(Theorem 1.4 of \citet{chen2020noisy}}) Let $\bX$ be rank-r and $\mu$-incoherent with a condition number $\kappa$. Suppose Assumption 1 holds and take $\lambda=C_\lambda \sigma \sqrt{n p}$ in \eqref{eq:opt} for some large enough constant $C_\lambda>0$. Assume the sample size obeys $n^2 p \geq C \kappa^4 \mu^2 r^2 n \log ^3 n$ for some sufficiently large constant $C>0$, and the noise satisfies $\sigma \sqrt{\frac{n}{p}} \leq c \frac{\sigma_{\min }}{\sqrt{\kappa^4 \mu r \log n}}$ for some sufficiently small constant $c>0$. Then with probability exceeding $1-O\left(n^{-3}\right)$,
1. any minimizer $\bZ_{\mathrm{cvx}}$ of (3) obeys
\begin{itemize}
    \item (11a) $\quad\left\|\bZ_{\mathrm{cvx}}-\bX\right\|_{\mathrm{F}} \lesssim \kappa \frac{\sigma}{\sigma_{\min }} \sqrt{\frac{n}{p}}\left\|\bX\right\|_{\mathrm{F}}$,
    \item (11b) $\quad\left\|\bZ_{\mathrm{cvx}}-\bX\right\|_{\infty} \lesssim \sqrt{\kappa^3 \mu r} \cdot \frac{\sigma}{\sigma_{\min }} \sqrt{\frac{n \log n}{p}}\left\|\bX\right\|_{\infty}$,
    \item (11c) $\quad\left\|\bZ_{\mathrm{cvx}}-\bX\right\| \lesssim \frac{\sigma}{\sigma_{\min }} \sqrt{\frac{n}{p}}\left\|\bX\right\|$
\end{itemize}
\end{theorem}
The $p$ denotes the proportion of arms in the noisy $\oX$ matrix. 

\smnote{They probably assume that $\bSigma_* = \bI$}

This naturally gives us the following explore then commit algorithm as follows:
% \begin{algorithm}[!tbh]
% \caption{Noisy Experimental Design (\ned)}
% \label{alg:linear-bandit}
% \begin{algorithmic}[1]
% \State \textbf{Input:} Finite set of actions $\A$,  budget $n$.
% \State Conduct E-optimal design exploration for $\Gamma=\sqrt{n}$ timesteps 
% \begin{align*}
%     \lambda^E_* = \min_{\boldsymbol{\lambda} \in \triangle_{\mathcal{X}}}\left\|\left(\sum_{i=1}^a \lambda\left(\ox_i\right) \ox_i \ox_i^{\top}\right)^{-1}\right\|
% \end{align*}
% where $\ox_i$ are the noisy features. 
% \State Estimate $\bX$ using \eqref{eq:opt} as follows:
% \begin{align*}
%     \bZ_{\mathrm{cvx}} = \underset{\bZ \in \mathbb{R}^{n \times d}}{\operatorname{minimize}} \quad  \frac{1}{2} \sum_{(i, j) \in \Omega}\left(Z_{i j}-\oX_{i j}\right)^2+\lambda\|\bZ\|_*
% \end{align*}
% Set $\widehat{\bX} = \bZ_{\mathrm{cvx}}$. 
% \State For $n-\Gamma$ timesteps implement the RAGE algorithm \citep{fiez2019sequential} which conducts the G-optimal design
% \begin{align*}
% \lambda_t^{G,*} \leftarrow \arg \min _{\lambda \in \Delta_{\mathcal{X}}} \max _{y \in \mathcal{Y}\left(\widehat{\mathcal{Z}}_t\right)}\|y\|_{\left(\sum_{x \in \mathcal{X}} \lambda_x \wx \wx^{\top}\right)^{-1}}^2
% \end{align*}
% \State \textbf{Output:} The optimal arm.
% \end{algorithmic}
% \end{algorithm}


\newpage
\section{Oracle Optimal Design under Persistent noise}

Let us consider an oracle that knows the injected noise $\bSigma$ but not the $\theta_*$.
Let the true feature matrix be denoted by $\bX\in\R^{A\times d}$. This matrix is corrupted by the persistent noise $\bSigma \in\R^{A\times d}$ such that $\bSigma = [\bz(1), \bz(2), \ldots, \bz(A)]$. So $\bz(a)\in\R^d$ is the corruption of arm $\bx(a)$. This is fixed for all round $n$. The observed corrupted matrix at round $t$ is given by
\begin{align*}
    \oX = \bX + \bSigma
\end{align*}
Let the oracle sample for $n$ rounds and create the matrix $\oX_n = [\ox_1, \ox_2, \ldots, \ox_n] \in \R^{n\times d}$ where $\ox_i = \bx_i + \bz_i$. Let the observed reward be $\bY_n = [Y_1, Y_2, \ldots, Y_n]\in \R^n$. Then let the corrupted estimate be
\begin{align*}
    \wtheta^e_n = (\oX_n^\top\oX_n)^{-1}\oX_n^\top\bY_n
\end{align*}
where, $\oX_n = \bX_n + \bSigma_n$ and $\bX_n = [\bx_1, \bx_2, \ldots, \bx_n] \in \R^{n\times d}$ are the stacked true features, $\bSigma_n = [\bz_1, \bz_2, \ldots, \bz_n]$ are the stacked persistent noise matrix. Let us consider the metric
\begin{align*}
    \E_{\D}&\left[\|\wtheta^e_n - \btheta_*\|^2_2\right] = \E_{\D}\left[\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top\bY_n - \btheta_*\|^2_2\right] = \E_{\D}\left[\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top\left(\bX_n\btheta_* + \eta\right) - \btheta_*\|^2_2\right]\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &= \E_{\D}\left[\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top\bX_n\btheta_* + (\oX_n^\top\oX_n)^{-1}\oX_n^\top\eta - \btheta_*\|^2_2\right]\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &\overset{(a)}{=} \E_{\D}\left[\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top(\oX_n-\bSigma_n)\btheta_* + (\oX_n^\top\oX_n)^{-1}\oX_n^\top\eta - \btheta_*\|^2_2\right]\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &= \E_{\D}\left[\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top\eta - (\oX_n^\top\oX_n)^{-1}\oX_n^\top\bSigma_n\btheta_*\|^2_2\right]\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &\overset{(b)}{=} \E_{\D}\left[\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top\bSigma_n\btheta_*\|^2_2\right]+ \E_{\D}\left[\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top\eta \|^2_2\right] \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &\qquad - 2\E_{\D}\left[\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top\bSigma_n\btheta_*\|\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top\eta\|\right]\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &\overset{(c)}{=} \E_{\D}\left[\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top\bSigma_n\btheta_*\|^2_2\right]+ \E_{\D}\left[\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top\eta \|^2_2\right] \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &\qquad - 2\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top\bSigma_n\btheta_*\|\E_{\D}\left[\|(\oX_n^\top\oX_n)^{-1}\oX_n^\top\eta\|\right]\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &\overset{(d)}{=} \E_{\D}\left[\Tr\left((\oX_n^\top\oX_n)^{-1}\oX_n^\top\bSigma_n\btheta_*(\bSigma_n\btheta_*)^\top\oX_n(\oX_n^\top\oX_n)^{-1}\right)\right]+ \E_{\D}\left[\Tr\left((\oX_n^\top\oX_n)^{-1}\oX_n^\top\eta\eta^\top\oX_n(\oX_n^\top\oX_n)^{-1}\right) \right] \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &= \E_{\D}\left[\Tr\left((\oX_n^\top\oX_n)^{-1}\oX_n^\top\bSigma_n\btheta_*(\bSigma_n\btheta_*)^\top\oX_n(\oX_n^\top\oX_n)^{-1}\right)\right]+ \Tr\left((\oX_n^\top\oX_n)^{-1}\oX_n^\top\E_{\D}\left[\eta\eta^\top\right]\oX_n(\oX_n^\top\oX_n)^{-1}\right) \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &\overset{(e)}{=} \E_{\D}\left[\Tr\left((\oX_n^\top\oX_n)^{-1}\oX_n^\top\bSigma_n\btheta_*(\bSigma_n\btheta_*)^\top\oX_n(\oX_n^\top\oX_n)^{-1}\right)\right]+ \Tr\left((\oX_n^\top\oX_n)^{-1}\right) \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    &\overset{(f)}{\leq} c^2\Tr\left((\oX_n^\top\oX_n)^{-1}\right)+ \Tr\left((\oX_n^\top\oX_n)^{-1}\right) = (1+c^2)\Tr\left((\oX_n^\top\oX_n)^{-1}\right)
\end{align*}
where, $(a)$ follows as $\oX_n = \bX_n - \bSigma_n$, $(b)$ follows as $\|\mathbf{a} - \mathbf{b}\|^2_2 = \|\mathbf{a}\|^2_2 + \|\mathbf{b}\|^2_2 - 2\|\mathbf{a}\|\|\mathbf{b}\|$. $(c)$ follows as the expectation is over noise, $(d)$ follows as $\E_\D[\eta] = \mathbf{0}$.The $(e)$ follows as $\E_{\D}[\eta\eta^\top] = \bI$. 
% and we denote $\bSigma_{\btheta_*} = \bSigma_n\btheta_*\in\R^d$. 


If we assume that the persistent noise is such that 
$\bSigma\btheta_*(\bSigma\btheta_*)^\top = \dfrac{c \bI}{n}$ for some constant $c>0$. Then we can show that
\begin{align*}
    \bSigma_n\btheta_*(\bSigma_n\btheta_*)^\top 
    = n^2\bSigma\btheta_*(\bSigma\btheta_*)^\top
    % \leq n^2\left(\frac{c\be}{n}\right)\left(\frac{c\be}{n}\right)^\top 
    =  c^2\bI
\end{align*}
% for some constant $c>0$. 
Then $(f)$ follows. So minimizing the quantity $\E_{\D}\left[\|\wtheta^e_n - \btheta_*\|^2_2\right]$ is equivalent to minimizing its upper bound the 
\begin{align*}
\Tr\left((\oX_n^\top\oX_n)^{-1}\right) = \Tr\left(\left(\sum_{t=1}^n\oX_t^\top\oX_t\right)^{-1}\right) = \dfrac{1}{n}\min_{\bp}\Tr\left(\left(\sum_{a=1}^A\bp(a)\left(\bx(a)+\bz(a)\right)\left(\bx(a)+\bz(a)\right)^\top\right)^{-1}\right)
\end{align*}
which lead to the A-optimal design.

==> pure_exp_bi.tex <==
In this section, we consider pure exploration in a single-task bi-linear bandit setting as a warm-up to the main goal of learning representation for multi-task bi-linear bandits. %\citep{jun2019bilinear,lu2021low,kang2022efficient}.
%
We first recall the single-task bilinear bandit setting as follows: At every round $t=1,2,\ldots$ the learner observes the reward $r_t = \bx_t^\top\bTheta_*\bz_t + \eta_t$ where the low rank hidden parameter $\bTheta_*\in\R^{d_1\times d_2}$ is unknown to the learner, $\bx_t\in\R^{d_1}$, $\bz_t\in\R^{d_2}$ are visible to the learner, and $\eta_t$ is a $1$-sub-Gaussian noise. We assume that the matrix $\bTheta_*$ has a low rank $r$ which is known to the learner and $d_1, d_2 \gg r$.
%
Finally recall that the goal is to identify the optimal left and right arms $\bx_*, \bz_*$ with a minimum number of samples. In the following sections, we state how we can leverage the low-rank structure of $\bTheta_*$, the bilinear structure, and optimal design \citep{pukelsheim2006optimal} to come up with a pure exploration algorithm.

\vspace*{-0.5em}
\subsection{Estimating Subspaces and Reduction to Low Dimensional Linear Bandits}
\vspace*{-0.5em}
\label{sec:low-dim-single}
Our algorithm proceeds in stages. 
In the first stage, the goal is to estimate the row and column sub-spaces $\bTheta_*$. Then we can use these estimates of row and column sub-spaces to reduce the bilinear bandit problem in the original ambient dimension $p\coloneqq d_1d_2$ to a lower effective dimension $k\coloneqq (d_1 + d_2)r$. 
%
Let the learner sample the actions $\{\bx_s,\bz_s\}_{s=1}^{n_1}$ following the $E$-optimal design \citep{pukelsheim2006optimal,jun2019bilinear} for $n_1$ rounds and observe rewards $\{r_s\}_{s=1}^{n_1}$.
%
Let $\wTheta_{n_1}$ be an estimate $\bTheta_*$. We can get the estimate by solving the following well-defined regularized minimization problem with nuclear norm penalty:
%
\begin{align}
\wTheta_{n_1}=\argmin _{\bTheta \in \mathbb{R}^{d_1 \times d_2}} L_{n_1}(\bTheta)+\lambda_{n_1}\|\bTheta\|_{\mathrm{nuc}}, \quad L_{n_1}(\bTheta)=\langle\bTheta, \bTheta\rangle-\frac{2}{n_1} \sum_{s=1}^{n_1}\left\langle\tilde{\psi}_\nu\left(r_s \cdot Q\left(\bx_s\bz_s^\top\right)\right), \bTheta\right\rangle \label{eq:convex-prog}
\end{align}
where $Q(\cdot)$, $\tilde{\psi}_\nu(\cdot)$, are appropriate functions stated in  \Cref{def:score-func}, \ref{def:psi-tilde} respectively. The parameter  $\lambda_{n_1}$ is defined in \Cref{theorem:kang-low-rank}. Then 
%
using \Cref{theorem:kang-low-rank} for $n_1$ rounds we get with probability \ $(1-\delta)$ that 
% \begin{align*}
$\|\wTheta_{n_1}- \bTheta_*\|_F^2 \leq \tfrac{C_1 d_1 d_2 r \log (2(d_1+d_2)/\delta)}{n_1}$ for some constant $C_1 > 0$.
% \end{align*}

\textbf{Reduction to linear bandits:}  Recall that $\bTheta_*= \bU \bD_* \bV^{{\top}}$ is the SVD of $\bTheta_*$ (where $\bD_*$ is $r \times r$ diagonal). Let $\wU,\wV$ are estimates of $\bU,\bV$ respectively. Let $\wU^{\perp}$ and $\wV^{\perp}$ are the complementary subspace of $\wU$ and $\wV$ respectively. Let $\mathbf{H}=[\wU \wU^{\perp}]^{\top} \bTheta_*[\wV \wV^{\perp}]$ be a rotated version of $\bTheta_*$. Then we have $\bTheta_* =[\wU \wU^{\perp}] \mathbf{H}[\wV \wV^{\perp}]^{\top}$ and $\bx^{\top} \bTheta_* \mathbf{z}=([\wU \wU^{\perp}]^{\top} \bx)^{\top} \mathbf{H}([\wV \wV^{\perp}]^{\top} \mathbf{z})$.
% \begin{align*}
% % \bTheta_* & =\left[\wU \wU_{\perp}\right] \mathbf{H}\left[\wV \wV_{\perp}\right]^{\top} \quad \text { and } %\\
% % \bx^{\top} \bTheta_* \mathbf{z}=\left(\left[\wU \wU_{\perp}\right]^{\top} \bx\right)^{\top} \mathbf{H}\left(\left[\wV \wV_{\perp}\right]^{\top} \mathbf{z}\right) .
% \bTheta_* & =[\wU \wU^{\perp}] \mathbf{H}[\wV \wV^{\perp}]^{\top} \quad \text { and } \quad %\\
% \bx^{\top} \bTheta_* \mathbf{z}=([\wU \wU^{\perp}]^{\top} \bx)^{\top} \mathbf{H}([\wV \wV^{\perp}]^{\top} \mathbf{z}) .
% \end{align*}
%
Thus, the bilinear bandit problem with the unknown $\bTheta_*$ with arm sets $\X$ and $\Z$ is equivalent to the one with the unknown $\mathbf{H}$ with rotated arm sets 
\begin{align}
% \X^{\prime}=\left\{\bx^{\prime}=\left[\wU \wU_\perp\right]^{\top} \bx \mid \bx \in \X\right\}, \quad
% \Z^{\prime}= \left\{\bz^{\prime}=\left[\wV \wV_{\perp}\right]^{\top} \mathbf{z} \mid \bz \in \Z\right\}
\uX=\{\ux=[\wU \wU^\perp]^{\top} \bx \mid \bx \in \X\}, \quad
\uZ= \{\uz=[\wV \wV^{\perp}]^{\top} \mathbf{z} \mid \bz \in \Z\}. \label{eq:rotated-arm-set}
\end{align}
Observe now that this problem can be cast as a $d_1 d_2$-dimensional linear bandit problem by considering the unknown vector $\btheta^*=\vec(\mathbf{H})$. The difference is, however, that we have learned about the subspace of $\bTheta_*$ in stage 1. We define $\btheta^*$ to be a rearranged version of vec $(\mathbf{H})$ so that the last $\left(d_1-r\right) \cdot\left(d_2-r\right)$ dimensions of $\btheta^*$ are $H_{i j}$ for $i \in\left\{r+1, \ldots, d_1\right\}$ and $j \in\left\{r+1, \ldots, d_2\right\}$; that is, letting $k:=d_1 d_2-(d_1-r) \cdot(d_2-r)$,
\begin{align}
& \btheta_{1: k}^* \!\!=\!\!\left[\vec\left(\mathbf{H}_{1: r, 1: r}\right) ; \vec\left(\mathbf{H}_{r+1: d_1, 1: r}\right) ; \vec\left(\mathbf{H}_{1: r, r+1: d_2}\right)\right], %\\
 \btheta_{k+1: p}^*\!\!=\!\!\vec\left(\mathbf{H}_{r+1: d_1, r+1: d_2}\right) .\label{eq:rotate-theta-single}
\end{align}
So
%\begin{align*}
$\|\btheta_{k+1: p}^*\|_2^2 =
%\!\!=\!\!\sum_{i>r \wedge j>r} H_{i j}^2\!\!=\!\!\|
(\wU^{\perp})^{\top}(\bU \bD_* \bV^{\top}) \wV^{\perp}\|_F^2 %\\
 \leq\|(\wU^{\perp})^{\top} \bU\|_F^2\|\bD_*\|_2^2\|(\wV^{\perp})^{\top} \bV\|_F^2  \leq \tO(\frac{d_1 d_2 r}{n_1 }):=S_\ell^{\perp}$,
%\end{align*}
%\log (\frac{d_1+d_2}{\delta})
which implies $\|\btheta_{k+1: p}^{\star}\|_2=O\left(d_1d_2 r / n_1\right)$ by \Cref{theorem:kang-low-rank}. Crucially observe that we have now reduced the $d_1d_2$ dimensional linear bandit to $(d_1 + d_2)r$ dimensional linear bandit with \eqref{eq:rotated-arm-set}, \eqref{eq:rotate-theta-single}.

\vspace*{-1em}
\subsection{Optimal Design for Bilinear Bandits}
\label{sec:optimal-design-single}
\vspace*{-1em}
%
In stage $2$, we learn in the rotated arm set $\uX, \uZ$ defined in  \eqref{eq:rotated-arm-set}.
%
We introduce the optimal design for the rotated arm set $\uX, \uZ$. The optimal design has been previously studied in the linear bandit setting both for pure exploration \citep{soare2014best, fiez2019sequential, katz2020empirical, zhu2021pure} or regret minimization \citep{lattimore2020bandit, wagenmaker2021experimental}. However, if we simply apply the techniques of these papers then our sample complexity will scale with the ambient dimension $p \coloneqq d_1d_2$ instead of the effective dimension $k \coloneqq (d_1 + d_2)r$. Next, we show how we can leverage the effective dimension to construct a new optimal design for the bilinear bandits. 

% To leverage the low-rank structure of $\bTheta_*$, the learner first builds an estimate of $\bTheta_*$ in the first stage. 


% Following the work of \citet{kang2022efficient} we can show that 

Define the $\uw = [\ux_{1:d_1};\uz_{1:d_2}] \in\R^p$ that belong to the set $\ucW$. 
%
%
Let the observed features till round $n$ be denoted by $\uW_n \in \R^{n\times p}$, and $\br_n \in \R^n$ be the observed rewards.
%
Define the diagonal matrix $\bLambda$ as
\begin{align}
    \bLambda = \mathbf{diag}[\underbrace{\lambda,\ldots,\lambda}_{k},\underbrace{\lambda_\perp,\ldots,\lambda_\perp}_{p-k}] \label{eq:bLambda}
\end{align}
where, $\lambda^\perp \gg \lambda$. 
%
Deviating from \citet{soare2014best, fiez2019sequential} we construct a regularized least square estimator (similar to \citet{valko2014spectral}) at round $n$ as follows
\begin{align}
    \wtheta_n=\argmin_{\btheta\in\R^p} \frac{1}{2}\|\uW_n \btheta-\br_n\|_2^2+\frac{1}{2}\|\btheta\|_{\bLambda}^2. \label{eq:least-sq-reg}
\end{align}
One of the key features of this regularized least square estimator is that it forces the last $p-k$ components of $\wtheta_n$ to be very small (close to $0$) compared to the first $k$ components. Using a concentration lemma (to be proved later) we can show that for any $\by\in\R^p$:
% 
\begin{align*}
    |\by^{\top}(\wtheta_n-\btheta_*)| \leq\|\by\|_{\bV_n^{-1}} 2 \sqrt{14 \log (2 / \delta)}+\left\|\btheta_*\right\|_{\bLambda} \leq \|\by\|_{\bV_n^{-1}} \sqrt{56 B^2_* \log (2 / \delta)}
\end{align*}
where the co-variance matrix $\bV_{n} \coloneqq \sum_{s=1}^{n}\uw_s \uw_s^\top +  \bLambda$ and $B_*$ is defined in \Cref{prop:conc}.
% to be defined later. 
%
Now we want this to hold for all $\by \in \Y^*(\ucW)$, and so we need to union bound over $\W\supseteq\ucW$ replacing $\delta$ with $\delta /|\W|$.
%
Set $n=\left\lceil 56 B^2_* \rho^* \log (2|\W| / \delta)\right\rceil$ where $\rho^*$ is to be defined later. Then for the  allocation $2\left\lfloor\bb_{\uw}^* n\right\rfloor$ for each $\bb_{\uw} \in \W$, we have for each $\uw \in \ucW \backslash \uw_*$ that with probability at least $1-\delta$,
\begin{align*}
    (\uw_*-\uw)^{\top}\wtheta_n &\geq (\uw_*-\uw)^{\top}\btheta_* - \|\uw_*-\uw\|_{(\sum_{\uw\in\W} \lceil2n\bb^*_{\uw}\rceil\uw\ \uw^\top + 2n\bLambda/n )^{-1}} \sqrt{56 B^2_* \log (2 |\W| / \delta)}%\\
    %%%%%%%%%%%%%%%%%%%%%%%
\end{align*}
since for every $\uw_*-\uw\in\Y^*(\W)$ we have
\begin{align*}
    (\uw_*-\uw)^\top\big(2\sum_{\uw\in\W} \lceil n\bb^*_{\uw}\rceil\uw \ \uw^\top + 2n\bLambda/n \big)^{-1} (\uw_*-\uw)&\leq  \tfrac{1}{n}\|\uw_*-\uw\|^2_{(\sum_{\uw\in\W} \bb^*_{\uw}\uw\ \uw^\top + \bLambda/n )^{-1}} %\\
    %%%%%%%%%%%%%%%%%%
    \leq \tfrac{((\uw_*-\uw)^{\top}\btheta_*)^2}{\sqrt{56 B^2_* \log (2 |\W| / \delta)}}.
\end{align*}
The last inequality follows by plugging in the value of $n$ and $\rho^*$.
%
Hence to minimize the sample complexity $n$ we can re-arrange the above equation to show that
\begin{align*}
    n \geq \sqrt{56 B^2_* \log (2 |\W|/ \delta)} \max_{\uw\in\W\setminus\uw_*} \tfrac{\|\uw_*-\uw\|^2_{(\sum_{\uw\in\W} \bb^*_{\uw}\uw\ \uw^\top + \bLambda/n )^{-1}}}{(\uw_*-\uw)^{\top}\btheta_*}
\end{align*}
Hence, to minimize the sample complexity for the bilinear setting we need to sample according to
\begin{align}
    \bb^G_* = \argmin_{\bb}\max_{\uw} \tfrac{\|\uw_*-\uw\|^2_{(\sum_{\uw\in\W} \bb_{\uw}\uw\ \uw^\top + \bLambda/n )^{-1}}}{(\uw_*-\uw)^{\top}\btheta_*} \label{eq:bi-level-opt}
\end{align}
The key point to note from \eqref{eq:bi-level-opt} is that due to the estimation in the rotated arm space $\ucW$ we are guaranteed that the support of $\mathbf{supp}(\bb^G_*) \leq \widetilde{O}(k(k+1)/2)$ \citep{pukelsheim2006optimal}. On the other hand, if the G-optimal design of \citet{fiez2019sequential,katz2020empirical} are run in $d_1d_2$ dimension then the support of $\bb^G_*$ will scale with $d_1d_2$.
%
%
% Given this knowledge, the learner aims to levra 
% the key difference for the bilinear bandit setting lies in the analysis of the OLS estimation $\wtheta_t$ and the goal of reducing the 
% These papers use $D$ or $G$-optimal design to minimize sample complexity for pure exploration or minimize regret. These designs naturally arise in the pure exploration setting in the following way:
% Consider the OLS estimation $\wtheta_t = $
% However, the 
%
%
% \vspace*{-1em}
\subsection{Single Task Pure Exploration Algorithm}
\label{sec:pure-exp-single}
\vspace*{-0.7em}
%
Following the sampling rule derived for the bilinear bandits in \eqref{eq:bi-level-opt} we can devise a pure exploration algorithm for the bi-linear setting. We propose a multi-stage phase-based algorithm called \textbf{G}-\textbf{O}ptimal Design for \textbf{B}i\textbf{lin}ear Bandits (abbreviated as \gob). In the first stage, for every phase $\ell$ the 
\gob\ explores the low-rank sub-space to estimate the $\bTheta_*$ by sampling arms  according to the $E$-optimal design \citep{pukelsheim2006optimal,jun2019bilinear,du2023multi}.
%
To do this, \gob\ first vectorizes the $\bx,\bz$ into a new vector $\ow\in\R^{p}$ and then solves the $E$-optimal design in \eqref{eq:E-opt-single} (see Step 4).
%
Let the solution to the $E$-optimal design  at the $\ell$-th phase be denoted by $\bb^E_\ell$. Then \gob\ samples each $\ow$ for $\lceil \tau^E_\ell\bb^E_{\ell,\ow} \rceil$ times, where $\tau^E_\ell$ is the length of the $\ell$-th exploration phase (step 8). 
%
Following \citet{kang2022efficient} we set the length of $\tau^E_\ell = \widetilde{O}(\sqrt{d_1 d_2 r}/ S_r)$. Then \gob\ builds the estimation $\wTheta_{\ell}$ using \eqref{eq:convex-prog} (step 9). 


In the second stage, for phase $\ell$ we first rotate the arms using \eqref{eq:rotated-arm-set} as follows:
%
Let $\wTheta_{\ell} = \wU_\ell\wD_{\ell}\wV_{\ell}^\top$ be the SVD of $\wTheta_{\ell}$ in the $\ell$-th phase. Let $\wU^\ell_{\perp}$ and $\wV^\ell_{\perp}$ be orthonormal bases of the complementary subspaces of $\wU_\ell$ and $\wV_\ell$ respectively. Let $\X_\ell$ and $\Z_\ell$ be the active set of arms in phase $\ell$. Then rotate the arm sets s.t. $\uX_\ell=\{\ux=[\wU_\ell \wU_\ell^\perp]^{\top} \bx \mid \bx \in \X_\ell\}, 
\uZ_\ell = \{\uz=[\wV_\ell \wV_\ell^{\perp}]^{\top} \mathbf{z} \mid \bz \in \Z_\ell\}$. Let $\wH_\ell=[\wU_\ell \wU^\perp_\ell]^{\top} \wTheta_{\ell}[\wV_\ell \wV_\ell^{\perp}]$. Then define vectorized arm set so that the last $\left(d_1-r\right) \cdot\left(d_2-r\right)$ components are from the complementary subspaces as follows:
%
\begin{align}
% \uX_\ell&=\{\ux=[\wU \wU_\perp]^{\top} \bx \mid \bx \in \X_\ell\}, \quad
% \uZ_\ell = \{\uz=[\wV \wV_{\perp}]^{\top} \mathbf{z} \mid \bz \in \Z_\ell\}, \nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\ucW_\ell = \left\{\left[\vec\left(\ux_{1: r} \uz_{1: r}^{\top}\right) ; \vec\left(\ux_{r+1: d_1} \uz_{1: r}^{\top}\right) ; \vec\left(\ux_{1: r} \uz_{r+1: d_2}^{\top}\right) ; \vec\left(\ux_{r+1: d_1} \uz_{r+1: d_2}^{\top}\right)\right] \in \mathbb{R}^{d_1 d_2}: \ux \in \X^{\prime}, \uz \in \mathcal{Z}^{\prime}\right\}\nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\wtheta_{\ell, 1: k}\!\!=\!\![\vec(\wH_{\ell,1: r, 1: r}) ; \vec(\wH_{\ell,r+1: d_1, 1: r}) ; \vec(\wH_{\ell,1: r, r+1: d_2})], %\\
 \btheta_{\ell, k+1: p}\!\!=\!\!\vec(\wH_{\ell,r+1: d_1, r+1: d_2}).
\label{eq:rotated-arm-set-phase}
\end{align}


Then we run the $G$-optimal design on the arm set $\ucW_\ell$ following the \eqref{eq:bi-level-opt} but replace $\uw_*$ with $\uw'$ (since $\uw_*$ is not known).
%
Let the solution to the $G$-optimal design  at the $\ell$-th phase be denoted by $\bb^G_\ell$. Then \gob\ samples each $\uw\in\ucW_\ell$ for $\lceil \tau^G_\ell\bb^G_{\ell,\uw} \rceil$ times, where $\tau^G_\ell$ is the length of the $\ell$-th exploration phase. 
%
Let at the $\ell$-th phase the actions sampled be denoted by the matrix $\uW_\ell\in\R^{\tau^G_\ell\times p}$ and observe rewards $\mathbf{r}\in\R^{\tau^G_{m,\ell}\times p}$. Define the positive diagonal matrix $\bLambda_\ell$ according to \eqref{eq:bLambda}. 
%
Specifically, we define $\bLambda_\ell= \mathbf{diag}\left(\lambda, \ldots, \lambda, \lambda_\ell^{\perp}, \ldots, \lambda_\ell^{\perp}\right)$, where $\lambda$ occupies the first $k$ diagonal entries and $\lambda^\ell_{\perp} = 8k\log(1+\tau^G_{\ell-1}/\lambda)$ the last $p-k$ positions. Then build 
%
% Then the estimation of $\btheta_*$ be
%
\begin{align}
\wtheta_\ell=\arg \min_{\btheta} \frac{1}{2}\|\uW_\ell \btheta-\mathbf{r}\|_2^2+\frac{1}{2}\|\btheta\|_{\bLambda_\ell}^2
% =\left(\bLambda_\ell +\uW_\ell^{\top} \uW_\ell\right)^{-1} \uW_\ell^{\top} \bR_\ell 
\label{eq:btheta-phase}
\end{align}
%
Finally \gob\ eliminates sub-optimal arms to build the next phase active set $\ucW_\ell$ and stops when $|\ucW_\ell| = 1$. The full pseudo-code is given in \Cref{alg:bandit-pure}.



% \begin{algorithm}
% \caption{G-Optimal Design for Bilinear Bandits (\gob)}
% \label{alg:bandit-pure}
% \begin{algorithmic}[1]
% \State Input: arm set $\X,\Z$, time horizon $n$, exploration length $n_1$, rank $r$ of $\bTheta_*$, spectral bound $S_r$ of $\bTheta_*$, sampling distribution for stage 1: $D$; parameters for stage $2: S, S_\ell^{\perp} =  \frac{8d_1 d_2 r}{\tau^E_{\ell} S^2_{r}} \log \left(\frac{d_1+d_2}{\delta_\ell}\right), \lambda, \lambda_\ell^{\perp} = \tau^G_{\ell-1}/8(d_1+d_2)r\log(1+\frac{\tau^G_{\ell-1}}{\lambda})$. Let $p=d_1d_2$, $k=(d_1+d_2)r$.
% %
% \State Let $\ucW_1 \leftarrow \ucW, \ell \leftarrow 1$, $\tau^G_0 = \log (4\ell^2|\X| / \delta)$.
% \State Define 
% % $\bA^\ell_{\bb_x} \!\!=\!\! \sum_{\bx\in\X_\ell}\bb_x\bx\bx^\top + \bLambda_\ell$, 
% $\bLambda_\ell \coloneqq \mathbf{diag}[\underbrace{\lambda,\ldots,\lambda}_{k},\underbrace{\lambda_\ell^\perp,\ldots,\lambda_\ell^\perp}_{p-k}]$, $B^\ell_* \coloneqq \left(8\sqrt{\lambda S^2 +\lambda_\ell^{\perp} S^{(2),\perp}_{\ell}}\right)$ 
% \State Define a vectorized arm $\ow = \left[\bx_{1: d_1}; \bz_{1: d_2}\right]$ and $\ow\in\ocW$. Let $\tau^E_{\ell} = \frac{\sqrt{8d_1 d_2 r\log (4\ell^2|\W| / \delta_\ell)}}{S_{r}}$. Let the $E$-optimal design be
% \begin{align}
%     \bb^E_\ell = \argmin_{\bb \in \triangle_{\ocW}}\big\|\big(\sum_{\ow\in\ocW} \bb_{\ow}\ow \ \ow^\top\big)^{-1}\big\| \label{eq:E-opt-single}
% \end{align}
% %
% \While{$\left|\ucW_{\ell}\right|>1$}
% %
% \State $\epsilon_{\ell}=2^{-\ell}$
% %
% % \State Let $\wb_{\ell,x} = \argmax_{\bb} \log\frac{|\bA^\ell_{\bb_x}|}{|\bLambda|}$ as the solution to $D$-optimal design for $\overline{\bX}_\ell$.
% % Similarly get $\wb_{\ell,z} = \argmax_{\bb} \log\frac{|\bA^\ell_{\bb_z}|}{|\bLambda|}$ as the solution to $D$-optimal design for $\Z$.
% %
% % \State $\epsilon_{\ell}=2^{-\ell}$, 
% % $\tau^E_{\ell} = \frac{8B^\ell_*\rho^E_*\log (4\ell^2|\W| / \delta)}{\epsilon_\ell^2}$. 
% % Similarly define $\tau_{\ell_z} = \frac{8k\log(1+\frac{\tau_{\ell_z-1}}{\lambda})\log (4\ell^2|\Z| / \delta)}{\epsilon^2}\left(\sqrt{56 R^2 } + \sqrt{\lambda S^2 +\lambda_{\perp} S^2_{\perp}}\right)$
% %
% \State \textbf{(Stage 1:) Explore the Low-Rank Subspace}
% \State Pull arm $\ow \in \ocW$ exactly $\left\lceil\wb^E_{\ell, \ow} \tau^E_{\ell}\right\rceil$ times
% % Pull $\bx_t \in \overline{\X}$ according to $\lceil\wb_{\ell_x}\tau_{\ell_x}\rceil$ 
% % and $\lceil\wb_{\ell_z}\tau_{\ell_z}\rceil$ respectively 
% and observe rewards $r_t$, for $t=1, \ldots, \tau^E_{\ell}$.
% \State Compute $\wTheta_{\tau^E_{\ell}}$ using \eqref{eq:convex-prog}.
% % $=\arg \min _{\bTheta \in \mathbb{R}^{d_1 \times d_2}} L_{n_1}(\bTheta)+\lambda_{n_1}\|\bTheta\|_{\mathrm{nuc}}, \quad L_{n_1}(\bTheta)=\langle\bTheta, \bTheta\rangle-\frac{2}{n_1} \sum_{i=1}^{n_1}\left\langle\tilde{\psi}_\nu\left(y_i \cdot S\left(X_i\right)\right), \bTheta\right\rangle $.
% %
% \State \textbf{(Stage 2:) Reduction to low dimensional linear bandits}  
% \State Let the SVD of $\wTheta_{\ell} = \wU_\ell\wD_{\ell}\wV_{\ell}^\top$. Then rotate the arm sets following \eqref{eq:rotated-arm-set-phase} to build $\ucW$.
% %
% % : $\X^{\prime}_\ell=\left\{\left[\wU \wU_{\perp}\right]^{\top} \bx: \bx \in \X\right\}$ and $\Z^{\prime}_\ell=\left\{\left[\wV \wV_{\perp}\right]^{\top} \bz: \bz \in \Z\right\}$.
% % Define a vectorized arm set so that the last $\left(d_1-r\right) \cdot\left(d_2-r\right)$ components are from the complementary subspaces:
% % \begin{align*}
% % \X_\ell=\left\{\left[\vec\left(\bx_{1: r} \bz_{1: r}^{\top}\right) ; \vec\left(\bx_{r+1: d_1} \bz_{1: r}^{\top}\right) ; \vec\left(\bx_{1: r} \bz_{r+1: d_2}^{\top}\right) ; \vec\left(\bx_{r+1: d_1} \bz_{r+1: d_2}^{\top}\right)\right] \in \mathbb{R}^{d_1 d_2}: \bx \in \X^{\prime}, \bz \in \Z^{\prime}\right\} .
% % \end{align*}
% % %
% %
% \State Let $\wb^G_{\ell} = \argmin_{\bb_{\uw}}\max_{\uw,\uw'\in\ucW_\ell} \|\uw-\uw'\|^2_{(\sum_{\uw\in\ucW} \bb_{\uw}\uw\ \uw^\top + \bLambda_\ell/n )^{-1}}$. 
% %
% \State Define $\rho^G(\Y(\ucW_{\ell})) = \min_{\bb_{\uw}}\max_{\uw,\uw'\in\ucW_\ell} \|\uw-\uw'\|^2_{(\sum_{\uw\in\ucW} \bb_{\uw}\uw\ \uw^\top + \bLambda_\ell/n )^{-1}}$. 
% %
% \State Set 
% $\tau^G_{\ell} \!\!=\!\! \frac{8(B^\ell_*)^2\rho^G(\Y(\W_\ell))\log (4\ell^2|\W| / \delta)}{\epsilon_\ell^2}$. 
% %
% %
% Then pull arm $\uw \in \ucW$ exactly $\left\lceil\wb_{\ell, \uw} \tau^G_{\ell}\right\rceil$ times and \indent construct the least squares estimator $\wtheta_{\ell}$ using only the observations of this phase where $\wtheta_\ell$ \indent is defined in \eqref{eq:btheta-phase}. Note that $\wtheta_\ell$ is also rotated following \eqref{eq:rotated-arm-set-phase}.
% % =\argmin_{\btheta} \frac{1}{2}\|\uW_\ell \btheta-\br\|_2^2+\frac{1}{2}\|\btheta\|_{\bLambda_\ell}^2$
% \State Eliminate arms such that 
% %\begin{align*}
% $\ucW_{\ell+1} \leftarrow \ucW_{\ell} \backslash\left\{\uw \in \ucW_{\ell}: \max_{\uw^{\prime} \in \ucW_{\ell}}\left\langle \uw^{\prime}-\uw, \wtheta_{\ell}\right\rangle>2 \epsilon_{\ell}\right\}$
% % \end{align*}
% \State $\ell \leftarrow \ell+1$
% \EndWhile
% \State Output the arm in $\ucW_{\ell}$ and reshape to get the $\widehat{\bx}_*$ and $\widehat{\bz}_*$
% \end{algorithmic}
% \end{algorithm}





\subsection{Sample Complexity Analysis of single task \gob}

We now analyze the sample complexity of \gob. We first present the sample complexity theorem for single task \gob. 


\begin{customtheorem}{1}\textbf{(informal)}
\label{thm:single-task}
With probability at least $1 - \delta$, \gob\ returns the best arms $\bx_*$, $\bz_*$, and the number of samples used is bounded by
\begin{align*}
    \widetilde{O}\left(\tfrac{(d_1+d_2)r}{\Delta_{}^2} + \tfrac{\sqrt{d_1 d_2 r}}{S_r}\right)
\end{align*}
\end{customtheorem}

\begin{discussion}
\smnote{To be written}
\end{discussion}


\textbf{Proof (Overview) of \Cref{thm:single-task}:} \textbf{Step 1 (Subspace estimation in high dimension):} We denote the vectorized arms in high dimension as $\ow\in\ocW$. We run the $E$-optimal design to sample the arms in $\ocW$. Note that this $E$-optimal design satisfies the distribution assumption of \citet{kang2022efficient} which enables us to apply the \Cref{theorem:kang-low-rank}. This leads to $\|\wTheta_\ell - \bTheta_*\|_F^2 \leq \tfrac{C_1 d_1 d_2 r \log \left(2\left(d_1+d_2\right)/\delta\right)}{\tau^E_\ell}$ for some $C_1>0$. 
%
Also, note that in the first phase by setting $\tau^E_{\ell} = \tfrac{\sqrt{8d_1 d_2 r\log (4\ell^2|\W| / \delta)}}{S_{r}}$ and sampling each arm $\ow \in \ocW$ exactly $\lceil\wb^E_{\ell, \ow} \tau^E_{\ell}\rceil$ times we are guaranteed that $\|\btheta_{k+1: p}^*\|_2=O(d_1d_2 r / \tau^E_\ell)$ in the $\ell$-th phase.
%
Summing up over $\ell=1$ to $\left\lceil\log _2\left(4 \Delta^{-1}\right)\right\rceil$ we get that the total samples complexity of the first stage is bounded by $\widetilde{O}({\sqrt{d_1 d_2 r}}/{S_r})$.


\textbf{Step 2 (Control log determinant in low dimension):} We first rotate the arms $\ow\in\ocW$ in high dimension to get the low dimensional arms $\uw\in\ucW$ following \eqref{eq:rotated-arm-set-phase}. Then we begin the proof with the concentration inequality in \Cref{eq:conc-lemma-bilin-exp} which shows that with high probability in the $\ell$-th phase the $|\uw^{\top}\left(\wtheta_\ell-\btheta_*\right)| \leq2 \sqrt{14 \log (2 / \delta)}+\|\btheta_*\|_{\bLambda_\ell}$ (where $\wtheta_\ell$ is the rotated version in \eqref{eq:rotated-arm-set-phase}). 
%
Next, we prove a log determinant inequality 
% similar to \citet{abbasi2011improved} 
in \Cref{lemma:valko-lemma-effective-dim-exp} that shows $
\log \tfrac{\left|\mathbf{V}_\ell\right|}{|\bLambda_\ell|} \leq 8 k \log \left(1+{\tau^G_{\ell-1}}/{\lambda}\right)$ 
when $\lambda_\ell^{\perp}=\tfrac{\tau^G_{\ell-1}}{k \log \left(1+\tau^G_{\ell-1} / \lambda\right)}$. Diverging from the proof technique of \citet{valko2014spectral}, note that the log determinant is bounded in the RHS by $\tau^G_{\ell-1}$ instead of a fixed budget $n$. Also, note that we have the effective dimension $k$ in the RHS. 
%
The key step to prove \Cref{lemma:valko-lemma-effective-dim-exp} is to show that at every level $\ell$ with the definition of $\rho^G(\Y(\ucW_{\ell}))$ we have that $\rho^G(\Y(\ucW_{\ell}))\leq k\log\left(1 + \tfrac{\tau^G_\ell}{\lambda}\right) \leq 8k\log\left(1 + \tfrac{\tau^G_{\ell-1}}{\lambda}\right)$. 
%
This enables us to avoid a cyclical dependency in setting the value of $\tau^G_\ell$ and $\lambda_\ell^\perp$ in $\bLambda_\ell$ at the phase $\ell$.
%
This step also diverges from the linear bandit pure exploration proof technique of \citet{fiez2019sequential,katz2020empirical,jamieson2022interactive} as there is no parameter $\lambda_\ell^\perp$ to control during phase $\ell$, and the effective dimensions in those papers do not depend on phase length.


\textbf{Step 3 (Equivalence):} For any phase $\ell$, using Lemma 1 from \citet{fiez2019sequential} we can show that $ 1 \leq \rho^G(\Y(\ucW_{\ell})) \leq p / \gamma_{\Y}^2$ where, $\gamma_{\Y}=\max \{c>0: c \Y \subset \operatorname{conv}(\ucW \cup-\ucW)\}$ is the gauge norm of $\Y$ \citep{rockafellar2015convex}. Note that this is a worst-case dependence when $\rho^G(\Y(\ucW_{\ell}))$ scales with $p$. Substituting this value of $\rho^G(\Y(\ucW_{\ell}))$ in the definition of $\lambda_\ell^\perp$ we can show that $\bLambda_\ell$ does not depend on $\uw$ or $\by = \uw-\uw'$. Then following Theorem 21.1 in \citet{lattimore2020bandit}  we can show that the $G$-optimal design $\wb^G_\ell$ is equivalent to $D$-optimal design $\wb^D_\ell = \argmax_{\bb} \log \tfrac{\left|\sum_{\uw\in\ucW_\ell}\bb_{\uw}\uw\ \uw^\top + \bLambda_\ell\right|}{|\bLambda_\ell|}$. Then using a variation of the Frank-Wolfe algorithm \citep{jamieson2022interactive} with a  stopping time in \eqref{eq:stopping-condition} we can show the support $\wb^G_\ell$ or equivalently $\wb^D_\ell$ is bounded by at most $\frac{8k\log(1+{\tau^G_{\ell-1}}/{\lambda})(8k\log(1+{\tau^G_{\ell-1}}/{\lambda}) + 1)}{2}$. This is shown in \Cref{lemma:equivalence}.

\textbf{Step 4 (Phase length and Elimination):} Using the \Cref{lemma:equivalence}, concentration  \Cref{eq:conc-lemma-bilin-exp}, and using the log determinant inequality in \Cref{lemma:valko-lemma-effective-dim-exp} and \Cref{prop:conc} we show that the phase length in the second stage is given by $\tau^G_\ell = \tfrac{8(B^\ell_*)^2 \rho(\Y(\ucW_\ell))  \log \left(2|\W| / \delta\right)}{(\bx^\top(\wtheta_\ell-\btheta^*))^2}$. This is discussed in \Cref{dis:phase-length}. We also show in \Cref{lemma:elim} that setting this phase length and sampling each active arm in $\ucW_\ell$ exactly $\left\lceil\wb_{\ell, \uw} \tau^G_{\ell}\right\rceil$ results in the elimination of sub-optimal actions with high probability.


\textbf{Step 5 (Total Samples):} Finally we combine the samples of each phase $\tau^G_\ell$ from $\ell=1$ to $\left\lceil\log _2\left(4 \Delta^{-1}\right)\right\rceil$ and first show that the total samples in the second phase are bounded by $\frac{k}{\gamma_{\Y}^2} O(B^\ell_*\log (\frac{k\log_2( \Delta^{-1})|\ucW|}{\delta}) \lceil\log _2(\Delta^{-1})\rceil)$ where the effective dimension $k=(d_1+d_2)r$.
% Observe that this scales with the effective dimension $k$.
%
%Then we show that in the first phase by setting $\tau^E_{\ell} = \tfrac{\sqrt{8d_1 d_2 r\log (4\ell^2|\W| / \delta)}}{S^2_{r}}$ and sampling each arm $\ow \in \ocW$ exactly $\left\lceil\wb^E_{\ell, \ow} \tau^E_{\ell}\right\rceil$ times we are guaranteed that $\left\|\btheta_{k+1: p}^*\right\|_2=O\left(d_1d_2 r / \tau^E_\ell\right)$ in the $\ell$-th phase. We use \Cref{theorem:kang-low-rank} from \citet{kang2022efficient} to show this and guarantee that $\|\wTheta- \bTheta^*\|_F^2 \leq \tfrac{C_1 d_1 d_2 r \log \left(\frac{2\left(d_1+d_2\right)}{\delta}\right)}{\tau^E_\ell}$ for some $C_1>0$. 
%
%Summing up over $\ell=1$ to $\left\lceil\log _2\left(4 \Delta^{-1}\right)\right\rceil$ we get that the total samples complexity of the first stage is bounded by $\widetilde{O}\left(\dfrac{\sqrt{d_1 d_2 r}}{S^2_r}\right)$. 
%
The claim of the theorem follows by combining the sample complexity of the first and second stages. 

==> self_supervised.tex <==
\begin{enumerate}
    \item Offline dataset $\D$
    \item Self-supervised in the sense reward free learning
    \item Representation learning 
\end{enumerate}



There is a state space $\mathcal{S}$, an action space $\mathcal{A}$, a known feature mapping $\phi: \mathcal{S} \times \mathcal{A} \mapsto \mathbb{R}^d$ and an unknown transition probability $P$. Let $h\in[H]$ be the horizon such that the interaction terminates after $H$ timesteps. The expected reward of each state-action pair $(s, a) \in \mathcal{S} \times \mathcal{A}$ is generated by $\boldsymbol{\phi}(s, a)^{\top} \boldsymbol{\theta}_h$, where $\boldsymbol{\theta}_h=\bB \boldsymbol{w}_h$. Substituting this above we have that
$$
\boldsymbol{\phi}(s, a)^{\top} \boldsymbol{\theta}_h = \boldsymbol{\phi}(s, a)^{\top}\bB \boldsymbol{w}_h = \overline{\phi}(s, a)^{\top}\bw_h
$$
where, $\overline{\phi}(s, a)\in \R^k$. Think that $\boldsymbol{\phi}(s, a)$ is a high dimensional raw input image, and $\overline{\phi}(s, a)$ is the low dimensional representation such that $d \gg k$. 



% We can interpret the problem as that the states-action pair at an arbitrary horizon level $h$ share a low-dimensional representation $\bB^{\top} \phi(s, a) \in \mathbb{R}^k$. 


The learning process is divided into two phase, 1) the exploration phase is when one does not have access to the reward function. 2) Planning phase when one has access to the reward function. Finally, the agent aims to identify an $\varepsilon$-optimal policy (i.e., a mapping $\mathcal{S} \mapsto \mathcal{A}$ that gives suboptimality within $\varepsilon$ ) for each task with confidence $1-\delta$, while minimizing the number of samples used.


Additionally, the agent has access to offline dataset $\D = \cup_{k=1}^K\{s^k_h,a^k_h,s^k_{h+1}\}_{h=1}^H$ for an arbitrary number of episodes $k=1$ to $K$ during the exploration phase. Observe that the dataset consists of no reward. However, the agent can use this information to construct a transition probability estimate $\wP$. 





\begin{assumption}
$\operatorname{MDP}(\mathcal{S}, \mathcal{A}, \mathrm{H}, P, \mathrm{r})$ is a linear (or Low rank?) MDP with a feature map $\phi: \mathcal{S} \times$ $\mathcal{A} \rightarrow \mathbb{R}^d$, if for any $h \in[H]$, there exist $d$ unknown (signed) measures $\mu_h=\left(\mu_h^{(1)}, \ldots, \mu_h^{(k)}\right)$ over $\mathcal{S}$ and an unknown vector $\boldsymbol{\theta}_h \in \mathbb{R}^d$, such that for any $(x, a) \in \mathcal{S} \times \mathcal{A}$, we have
\begin{align*}
\mathbb{P}_h(\cdot \mid s, a) &= \left\langle \phi(s, a)^\top\bB, \boldsymbol{\mu}_h(\cdot)\right\rangle = \left\langle\overline{\phi}(s, a), \boldsymbol{\mu}_h(\cdot)\right\rangle \\
%%%%%%%%%%%%%%%%%%%
r_h(s, a) & =\left\langle\phi(s, a)^\top\bB, \bw_h\right\rangle = \left\langle\overline{\phi}(s, a), \bw_h\right\rangle   .
\end{align*}
\end{assumption}
Note that diverging from the Jin et al. (2019, 2020)  Linear MDP definition, the signed measure $\mu$ is in $\R^k$, and the reward is defined with respect to $\bw_h$.

\smnote{Connection with Low-rank MDP, Block MDP?}

\smnote{Let's try to do model-free learning. And also see how we can use bi-simulation metrics.}


\newpage



\begin{assumption}\textbf{(Linear MDP with noisy feature)}
$\operatorname{MDP}(\mathcal{S}, \mathcal{A}, \mathrm{H}, P, \mathrm{r})$ is a linear MDP with a feature map $\phi: \mathcal{S} \times$ $\mathcal{A} \rightarrow \mathbb{R}^d$, if for any $h \in[H]$, there exist $d$ unknown (signed) measures $\mu_h=\left(\mu_h^{(1)}, \ldots, \mu_h^{(k)}\right)$ over $\mathcal{S}$ and an unknown vector $\boldsymbol{\theta}_h \in \mathbb{R}^d$, such that for any $(x, a) \in \mathcal{S} \times \mathcal{A}$, we have
\begin{align*}
\mathbb{P}_h(\cdot \mid s, a) &= \left\langle \overline{\phi}(s, a), \boldsymbol{\mu}_h(\cdot)\right\rangle \\
%%%%%%%%%%%%%%%%%%%
% \|\mathbb{P}_h(\cdot \mid s, a) - \left\langle \overline{\phi}(s, a), \boldsymbol{\mu}_h(\cdot)\right\rangle\|_{TV}\leq \xi \\
%%%%%%%%%%%%%%%%%%%
r_h(s, a) & =\left\langle\overline{\phi}(s,a),\bw_h\right\rangle.
\end{align*}
where, $\overline{\phi}(s,a) = \phi(s,a) + \eta_h$ where $\eta_h\sim \SG(0_{d\times 1}, \bSigma_h)$ and $\bSigma_h\in\R^{d\times d}$.
\end{assumption}
\smnote{First fix the noise,then calculate $\overline{\phi}$}

How to make this a distribution?


Plugging this back we get
\begin{align*}
    & \underbrace{\mathbb{P}_h(\cdot \mid s, a)}_{\text{Valid distribution}} = \left\langle \overline{\phi}(s, a), \boldsymbol{\mu}_h(\cdot)\right\rangle = \left\langle  \phi(s,a) + \eta_h, \boldsymbol{\mu}_h(\cdot)\right\rangle = \underbrace{\left\langle  \phi(s,a), \boldsymbol{\mu}_h(\cdot)\right\rangle}_{\text{Valid distribution}} + \left\langle \eta_h, \boldsymbol{\mu}_h(\cdot)\right\rangle\\
    %%%%%%%%%%%%%%%%%%%%%
    \implies & \|\underbrace{\mathbb{P}_h(\cdot \mid s, a)}_{\text{Valid distribution}} - \underbrace{\left\langle  \phi(s,a), \boldsymbol{\mu}_h(\cdot)\right\rangle }_{\text{Valid distribution}}\|_{TV} \leq \left\langle \eta_h, \boldsymbol{\mu}_h(\cdot)\right\rangle
\end{align*}
Note that if 
\begin{align*}
   \eta_h^\top \boldsymbol{\mu}_h(\cdot)\sim \mathrm{Ber}(p)
\end{align*}
where, $p=\boldsymbol{\mu}_h(.)^\top\bSigma_d\boldsymbol{\mu}_h(.) \leq 1$ then we have that 
\begin{align*}
    \|\underbrace{\mathbb{P}_h(\cdot \mid s, a)}_{\text{Valid distribution}} - \underbrace{\left\langle  \phi(s,a), \boldsymbol{\mu}_h(\cdot)\right\rangle }_{\text{Valid distribution}}\|_{TV} \leq \left\langle \eta_h, \boldsymbol{\mu}_h(\cdot)\right\rangle
\end{align*}
a valid distance as $\left\langle \eta_h, \boldsymbol{\mu}_h(\cdot)\right\rangle\in [0,1]$. This definition also 
% \begin{align*}
%     \eta_h\sim\SG(0_d,\bSigma_d) \implies\eta_h^\top \boldsymbol{\mu}_h(\cdot)\sim\SG(0_d,\boldsymbol{\mu}_h^\top\bSigma_d\boldsymbol{\mu}_h)
% \end{align*}
gives rise to heteroscedasticity as well. Also note that Bernoulli is a bounded distribution, and all bounded distributions are sub-Gaussian. So we can use sub-Gaussian concentration inequalities for free as we did for SPEED.






\begin{assumption}\textbf{(Linear MDP with noisy feature)}
$\operatorname{MDP}(\mathcal{S}, \mathcal{A}, \mathrm{H}, P, \mathrm{r})$ is a linear MDP with a feature map $\phi: \mathcal{S} \times$ $\mathcal{A} \rightarrow \mathbb{R}^d$, if for any $h \in[H]$, there exist $d$ unknown (signed) measures $\mu_h=\left(\mu_h^{(1)}, \ldots, \mu_h^{(k)}\right)$ over $\mathcal{S}$ and an unknown vector $\boldsymbol{\theta}_h \in \mathbb{R}^d$, such that for any $(x, a) \in \mathcal{S} \times \mathcal{A}$, we have
\begin{align*}
\mathbb{P}_h(\cdot \mid s, a) &= \E_{\D}\left[\left\langle \overline{\phi}(s, a), \boldsymbol{\mu}_h(\cdot)\right\rangle\right] \\
%%%%%%%%%%%%%%%%%%%%%
r_h(s, a) & =\E_{\D}\left[\left\langle\overline{\phi}(s,a),\bw_h\right\rangle\right]
\end{align*}
where, $\overline{\phi}(s,a) = \phi(s,a) + \eta_h$ where $\eta_h\sim \SG(0_{d\times 1}, \bSigma_h)$ and $\bSigma_h\in\R^{d\times d}$.
\end{assumption}
Now observe that
\begin{align*}
    \mathbb{P}_h(\cdot \mid s, a) = \E_{\D}\left[\left\langle \overline{\phi}(s, a), \boldsymbol{\mu}_h(\cdot)\right\rangle\right] = \E_{\D}\left[\underbrace{\left\langle  \phi(s,a), \boldsymbol{\mu}_h(\cdot)\right\rangle}_{\text{Valid distribution}} + \left\langle \eta_h, \boldsymbol{\mu}_h(\cdot)\right\rangle\right] &= \underbrace{\left\langle  \phi(s,a), \boldsymbol{\mu}_h(\cdot)\right\rangle}_{\text{Valid distribution}} +  \E_{\D}\left[\left\langle \eta_h, \boldsymbol{\mu}_h(\cdot)\right\rangle\right]\\
    %%%%%%%%%%%%%%
    &= \underbrace{\left\langle  \phi(s,a), \boldsymbol{\mu}_h(\cdot)\right\rangle}_{\text{Valid distribution}}
\end{align*}
\newpage 

==> tmp.tex <==
We study the multiclass classification (CSMC) problems with $K$ classes, where there is an instance space $\mathcal{X}$, a label space $\mathcal{Y}=\{1, \ldots, K\}$, and a distribution $\mathcal{D}$ supported on $\mathcal{X} \times[0,1]^K$.
%
Let $\mathcal{G} \triangleq\{g: \mathcal{X} \mapsto[0,1]\}$ denote a set of base regressors and let $\mathcal{F} \triangleq \mathcal{G}^K$ denote a set of vector regressors where the $y^{\text {th }}$ coordinate of $f \in \mathcal{F}$ is written as $f(\cdot ; y)$. The set of classifiers under consideration is $\mathcal{H} \triangleq\left\{h_f \mid f \in \mathcal{F}\right\}$ where each $f$ defines a classifier $h_f: \mathcal{X} \mapsto \mathcal{Y}$ by
\begin{align*}
h_f(x) \triangleq \underset{y}{\operatorname{argmin}} f(x ; y) .
\end{align*}



% When example $i \in[n]$ is queried, the agent receives label $Y_i \sim \operatorname{Bern}\left(\eta_i\right)$ where $\eta=\left(\eta_i\right)_{i=1}^n \in[0,1]^n$. 

We define the error of a hypothesis $h_f \in \mathcal{H}$ on the pool of examples as given by
\begin{align*}
\operatorname{err}(h_f) & =\frac{1}{n} \sum_{i=1}^n \mathbb{P}\left(Y_i \neq h_f\left(x_i\right)\right) =  \frac{1}{n} \sum_{i=1}^n \ell\left(Y_i, h_f\left(x_i\right)\right)
% \\
% & =\frac{1}{n} \sum_{i \in[n]} \eta_i\left(1-h\left(x_i\right)\right)+\left(1-\eta_i\right) h\left(x_i\right) .
\end{align*}
where, when example $i \in[n]$ is queried, the label $Y_i$ is the true label.

Consider the optimal sampling distribution over our pool of unlabeled examples $[n]$. For an arbitrary distribution $\lambda \in \triangle_n:=\left\{p \in \mathbb{R}^n: p_i \geq 0, \forall i \in\right.$ $\left.[n] ; \sum_{i=1}^n p_i=1\right\}$ suppose we sampled $I_1, \cdots, I_t \sim \lambda$ and then observed $y_s$ for each $s \in[t]$. 
%
% We consider a squared loss function like
% \begin{align*}
%     \ell(h\left(x_{I_s}\right),y_s) = (h\left(x_{I_s}\right) - y_s)^2
% \end{align*}
%
Then an unbiased natural estimator for the error of a classifier $h_f \in \mathcal{H}$ defined by $\operatorname{err}(h_f)$ is given by
\begin{align*}
\widetilde{\operatorname{err}}(h_f)=\frac{1}{t} \sum_{s=1}^t \frac{1 / n}{\lambda_{I_s}} \mathbb{I}\left\{h_f\left(x_{I_s}\right) \neq y_s\right\}, \qquad \widetilde{\operatorname{err}}(h_f)=\frac{1}{t} \sum_{s=1}^t \frac{1 / n}{\lambda_{I_s}} \ell(h_f\left(x_{I_s}\right), y_s) = \frac{1}{t} \sum_{s=1}^t \frac{1 / n}{\lambda_{I_s}} (h_f\left(x_{I_s}\right) - y_s)^2
\end{align*}
Indeed, by i.i.d. sampling from $\lambda$, we have for any $s \in[t]$
\begin{align*}
\mathbb{E}[\widetilde{\operatorname{err}}(h_f))] & =\mathbb{E}\left[\frac{1 / n}{\lambda_{I_s}}  \ell(h_f\left(x_{I_s}\right), y_s)\right] \\
& =\sum_{i=1}^n \mathbb{P}\left(I_s=i\right) \frac{1 / n}{\lambda_i} \mathbb{E}\left[ \ell(h_f\left(x_{I_s}\right), y_s) \mid I_s=i\right] \\
& =\frac{1}{n} \sum_{i=1}^n \mathbb{E}\left[ \ell(h_f\left(x_{I_s}\right), y_s)\right]=\operatorname{err}(h_f)
\end{align*}
since by definition, $\mathbb{P}\left(I_s=i\right)=\lambda_i$. Likewise, an estimator for the excess risk is given by
$$
\begin{aligned}
& \widetilde{\operatorname{err}}(h_f)-\widetilde{\operatorname{err}}\left(h_*\right)=  \quad \frac{1}{t} \sum_{s=1}^t \frac{1 / n}{\lambda_i}\left(\ell(h_f\left(x_{I_s}\right), y_s)-\ell(h_*\left(x_{I_s}\right), y_s)\right)\\
%%%%%%%%%%%%
&\widetilde{\operatorname{err}}(h_f)- \operatorname{err}(h_*) +  \operatorname{err}(h_*) - \widetilde{\operatorname{err}}\left(h_*\right)=  \quad \frac{1}{t} \sum_{s=1}^t \frac{1 / n}{\lambda_i}\left(\ell(h_f\left(x_{I_s}\right), y_s)-\ell(h_*\left(x_{I_s}\right), y_s)\right)
\end{aligned}
$$
We can show that the variance of $\widetilde{\operatorname{err}}(h_f)-$ $\widetilde{\operatorname{err}}\left(h_*\right)$ is upper bounded by $\frac{1}{n} \sum_{i=1}^n \frac{1}{\lambda_i n^2} \mathbb{I}\left\{h_*\left(x_i\right) \neq\right.$ $\left.h_f\left(x_i\right)\right\}$, using the upper bound $\mathbb{I}\left\{h_f\left(x_I\right) \neq y_s\right\}-$ $\left.\mathbb{I}\left\{h_*\left(x_I\right) \neq y_s\right\}\right) \leq \mathbb{I}\left\{h_*\left(x_I\right) \neq h_f\left(x_I\right)\right\}$. Applying Bernstein's inequality (and ignoring the $1 / t$ term) with probability at least $1-\delta$
%
\begin{align*}
& \left|\widetilde{\operatorname{err}}(h_f)-\widetilde{\operatorname{err}}\left(h_*\right)-\left(\operatorname{err}(h_f)-\operatorname{err}\left(h_*\right)\right)\right| \lesssim 
 \sqrt{\frac{\sum_{i=1}^n \frac{1}{\lambda_i n^2} \mathbb{I}\left\{h_*\left(x_i\right) \neq h_f\left(x_i\right)\right\} \log \left(\left|\mathcal{H}\right| / \delta\right)}{t}}
\end{align*}
%
This then suggests that to estimate the excess error of this particular $h$ with probability at least $1-\delta$, it suffices to take $t$ large enough to make the RHS of the above eq less than $\epsilon$. To upper bound the excess risk of every $h \in \mathcal{H}$ simultaneously, it suffices to take $t \geq$ $\sup _{h \in \mathcal{H}} \frac{\sum_{i=1}^n \frac{1}{\lambda_i n^2} \mathbb{I}\left\{h_*\left(x_i\right) \neq h\left(x_i\right)\right\}}{\max \left\{\epsilon^2,\left(\operatorname{err}(h)-\operatorname{err}\left(h_*\right)\right)^2\right\}} \log (|\mathcal{H}| / \delta)$. If we seek to minimize the total number of observations, we simply minimize over all $\lambda \in \triangle_n$, motivating the complexity measure:
\begin{align*}
\rho^*(\epsilon):=\inf _{\lambda \in \triangle_n} \sup _{h_f \in \mathcal{H} \backslash\left\{h_*\right\}} \frac{\sum_{i=1}^n \frac{1}{\lambda_i n^2} \mathbb{I}\left\{h_*\left(x_i\right) \neq h_f\left(x_i\right)\right\}}{\max \left(\operatorname{err}(h_f)-\operatorname{err}\left(h_*\right), \epsilon\right)^2} .
\end{align*}
Thus, we'd expect that if $t \geq \rho^*(\epsilon) \log (|\mathcal{H}| / \delta)$ samples are drawn from the $\lambda$ that minimizes $\rho^*(\epsilon)$, then $\widehat{h}=$ $\arg \min _{h_f \in \mathcal{H}} \widetilde{\operatorname{err}}(h_f)$ will be $\epsilon$-good.
